Meent: Differentiable Electromagnetic Simulator for Machine Learning

Electromagnetic (EM) simulation plays a crucial role in analyzing and designing devices with sub-wavelength scale structures such as solar cells, semiconductor devices, image sensors, future displays and integrated photonic devices. Specifically, optics problems such as estimating semiconductor device structures and designing nanophotonic devices provide intriguing research topics with far-reaching real world impact. Traditional algorithms for such tasks require iteratively refining parameters through simulations, which often yield sub-optimal results due to the high computational cost of both the algorithms and EM simulations. Machine learning (ML) emerged as a promising candidate to mitigate these challenges, and optics research community has increasingly adopted ML algorithms to obtain results surpassing classical methods across various tasks. To foster a synergistic collaboration between the optics and ML communities, it is essential to have an EM simulation software that is user-friendly for both research communities. To this end, we present Meent, an EM simulation software that employs rigorous coupled-wave analysis (RCWA). Developed in Python and equipped with automatic differentiation (AD) capabilities, Meent serves as a versatile platform for integrating ML into optics research and vice versa. To demonstrate its utility as a research platform, we present three applications of Meent: 1) generating a dataset for training neural operator, 2) serving as an environment for the reinforcement learning of nanophotonic device optimization, and 3) providing a solution for inverse problems with gradient-based optimizers. These applications highlight Meent's potential to advance both EM simulation and ML methodologies. The code is available at https://github.com/kc-ml2/meent with the MIT license to promote the cross-polinations of ideas among academic researchers and industry practitioners.

==> sections/applications/ocd-old.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{sections/applications/images/ocd-scheme.png}
    \caption{
        \textbf{Schematic Diagram Illustrating OCD via Spectrum Fitting.}
        The figure depicts the schematic representation of optical critical dimension (OCD) metrology using spectrum fitting. The diagram illustrates the key components of the approach, including the vector of design parameters ($\mathbf{\hat{\textit P}}$) obtained from the physical device, the set of spectra ($\mathbf{\hat{\textit S}}$) derived from these parameters, the synthesized spectra at iteration $\mathbf{\textit{i}}$ ($\mathbf{\textit{S}_\textit{i}}$), and the estimated design parameters at the corresponding iteration ($\mathbf{\textit{P}_\textit{i}}$). The methodology involves assessing the distance between the synthesized spectra and the ground truth spectra using a loss function, with subsequent updates to the design parameters to minimize this distance during each iteration.
    }
    \label{fig:ocd-scheme}
\end{figure}

RCWA finds one of its most successful applications in optical metrology within the semiconductor industry. It serves to estimate the dimensions of devices between process steps, thereby effectively monitoring excursions and maximizing yield for its non-destructive nature and high throughput capabilities.

A semiconductor device is a three-dimensional stack of layers, rendering direct measurement of parameters beneath the surface unfeasible without causing damage. This limitation is particularly critical in the context of high-volume manufacturing processes.
OCD offers a solution to this challenge by shifting (redirecting) the observation target from the physical device to its spectral characteristics, employing an indirect measurement approach. Consequently, OCD becomes an inverse problem: we deduce the dimensions of the structure in real space, which are the causal factors of spectrum shape, from observations (referred to as spectrum).
The solution involves a probabilistic and iterative process known as spectrum fitting. This necessitates optimization in continuous space, which can be achieved using Meent with Vector modeling, \cyp{which will be discussed in ...}.

Fig. \ref{fig:ocd-scheme} shows the process of finding solution using spectrum fitting. 

To simulate a real-world scenario where we have both the real device and its spectra, we first determine values for the ground truth, denoted as $\mathbf{\hat{\textit P}}$, and generate spectra $\mathbf{\hat{\textit S}}$ from a virtual structure defined by $\mathbf{\hat{\textit P}}$. The objective is to estimate $\mathbf{\hat{\textit P}}$ using $\mathbf{\hat{\textit S}}$, as direct measurement of $\mathbf{\hat{\textit P}}$ is not feasible. 
To achieve this, we initially create a virtual structure with limited prior knowledge provided by domain experts, and we randomly draw the initial parameters $\mathbf{\textit{P}_\textit{0}}$ from a suitable distribution. Subsequently, we generate $\mathbf{\textit{S}_\textit{0}}$ from $\mathbf{\textit{P}_\textit{0}}$.
We then employ a distance metric to quantify the discrepancy between the estimated and ground truth parameters. 
The process involves obtaining a loss value followed by backpropagation, which provides guidance on whether the elements of $\mathbf{\textit{P}_\textit{0}}$ should be adjusted upwards or downwards. This iterative process can be generalized using $\mathbf{\textit{P}_\textit{i}}$ and $\mathbf{\textit{S}_\textit{i}}$, where $\textit{i}$ denotes the iteration number.
As we keep iterating, $\mathbf{\textit{S}_\textit{i}}$ approaches $\mathbf{\hat{\textit S}}$ and presumably $\mathbf{\textit{P}_\textit{i}}$ approaches $\mathbf{\hat{\textit P}}$, where $\mathbf{\hat{\textit P}}$ is the parameter set we aim to find.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{sections/applications/images/ocd-scheme.png}
%     \caption{
%     % %% original
%     % \\~\\
%     % A scheme of OCD through spectrum fitting.
%     % $\mathbf{\hat{\textit P}}$ is a vector of design parameters from real device (ground truth in ML term), $\mathbf{\hat{\textit S}}$ is a set of spectrum (feature in ML) from $\mathbf{\hat{\textit P}}$, $\mathbf{\textit{S}_\textit{i}}$ is a set of synthesized spectrum at iteration $\mathbf{\textit{i}}$, and $\mathbf{\textit{P}_\textit{i}}$ is the estimated design parameter at iteration $\mathbf{\textit{i}}$.
%     % To find the dimension of $\mathbf{\hat{\textit P}}$, we measure the distance (loss function) between $\mathbf{\textit{S}_\textit{i}}$ and  $\mathbf{\hat{\textit S}}$, instead of $\mathbf{\textit{P}_\textit{i}}$ and $\mathbf{\hat{\textit P}}$, and update $\mathbf{\textit{P}_\textit{i}}$ to the direction that decreases the distance in iteration of $\mathbf{\textit{i}}$.\\~\\
%     \textbf{Schematic Diagram Illustrating OCD via Spectrum Fitting.}
%     The figure depicts the schematic representation of optical critical dimension (OCD) metrology using spectrum fitting. The diagram illustrates the key components of the approach, including the vector of design parameters ($\mathbf{\hat{\textit P}}$) obtained from the physical device, the set of spectra ($\mathbf{\hat{\textit S}}$) derived from these parameters, the synthesized spectra at iteration $\mathbf{\textit{i}}$ ($\mathbf{\textit{S}_\textit{i}}$), and the estimated design parameters at the corresponding iteration ($\mathbf{\textit{P}_\textit{i}}$). The methodology involves assessing the distance between the synthesized spectra and the ground truth spectra using a loss function, with subsequent updates to the design parameters to minimize this distance during each iteration.
%     }
%     \label{fig:ocd-scheme}
% \end{figure}

% % original
% % One of the most successful RCWA applications is its use in optical metrology in the semiconductor industry. It is used to estimate the dimensions of the device between the process steps, thereby monitoring excursion and maximizing the yield.

% % Among the methods, OCD is useful due to its non-destructive nature and high throughput.
% % Semiconductor device is a stack of multiple layers, that means any parameters beneath the surface cannot be directly measured (like photograph) without breaking it, which is unacceptable for high volume manufacturing.


% %% gpt 1)
% RCWA finds one of its most successful applications in optical metrology within the semiconductor industry. It serves to estimate the dimensions of devices between process steps, thereby effectively monitoring excursions and maximizing yield for its non-destructive nature and high throughput capabilities.

% %% gpt 2)
% % "One of the most successful applications of RCWA lies in optical metrology within the semiconductor industry. RCWA plays a crucial role in estimating the dimensions of semiconductor devices between process steps, facilitating the effective monitoring of excursions and maximizing of yield. This is primarily attributed to its non-destructive nature and high throughput capabilities. 


% % ----------------
% % original
% % Semiconductor device is a 3 dimensional stack of layers which make rendering direct measurement of parameters beneath the surface unfeasible without damage.
% % This limitation is particularly problematic in the context of high-volume manufacturing processes."

% % OCD, on the other hand, avoid this issue by change the target to observe - from real device to spectrum - i.e. indirect measurement. This makes OCD and inverse problem: we calculate from observations (called spectrum) the dimension of the structure in real space which is the causal factor of spectrum shape. The solution is found by probabilistic and iterative process called spectrum fitting. This requires optimization in continuous space, which can be done with Meent using Vector modeling.
% % ----------------
% % Here's the revised version for an academic journal:
% A semiconductor device is a three-dimensional stack of layers, rendering direct measurement of parameters beneath the surface unfeasible without causing damage. This limitation is particularly critical in the context of high-volume manufacturing processes.
% OCD offers a solution to this challenge by shifting (redirecting) the observation target from the physical device to its spectral characteristics, employing an indirect measurement approach. Consequently, OCD becomes an inverse problem: we deduce the dimensions of the structure in real space, which are the causal factors of spectrum shape, from observations (referred to as spectrum).
% The solution involves a probabilistic and iterative process known as spectrum fitting. This necessitates optimization in continuous space, which can be achieved using Meent with Vector modeling.
% % \paragraph{spectrum fitting}

% Fig. \ref{fig:ocd-scheme} shows the process of finding solution using spectrum fitting. 
% %% original
% % To mimic the situation that we have the real structure and its spectrum for the simulation experiments, we pick values for ground truth, $\mathbf{\hat{\textit P}}$, and make a spectrum $\mathbf{\hat{\textit S}}$ from the virtual structure having $\mathbf{\hat{\textit P}}$. 
% % Goal is to find $\mathbf{\hat{\textit P}}$ using $\mathbf{\hat{\textit S}}$ since $\mathbf{\hat{\textit P}}$ cannot be directly measured. 
% % 
% % To find these, virtual structure is created with vague prior knowledge by domain experts and the initial parameters $\mathbf{\textit{P}_\textit{0}}$ are drawn from any distribution. $\mathbf{\textit{S}_\textit{0}}$ is then generated from $\mathbf{\textit{P}_\textit{0}}$. 
% % 
% % Now we can use distance metric. Getting loss is followed by backpropagation that tell user that the element of $\mathbf{\textit{P}_\textit{0}}$ should be larger or smaller.
% % 
% % This can be generalized by $\mathbf{\textit{P}_\textit{i}}$ and $\mathbf{\textit{P}_\textit{i}}$ where $\textit{i}$ is the iteration. 
% % 
% % As keep iterating, $\mathbf{\textit{S}_\textit{i}}$ approaches to $\mathbf{\hat{\textit S}}$ and presumably $\mathbf{\textit{P}_\textit{i}}$ to $\mathbf{\hat{\textit P}}$, where $\mathbf{\hat{\textit P}}$ is what we want to find.
% % 
% % 
% % ----
% % 
% % chatgpt
% % Schematic Diagram Illustrating OCD Modeling via Spectrum Fitting.
% % A schematic representation for optical critical dimension metrology (OCD) using spectrum fitting is presented. $\mathbf{\hat{\textit P}}$ denotes the vector of design parameters from the physical device, referred to as the ground truth in the context of machine learning. $\mathbf{\hat{\textit S}}$ refers to a collection of spectra, considered as features in machine learning, derived from $\mathbf{\hat{\textit P}}$. $\mathbf{\textit{S}_\textit{i}}$ signifies a set of synthesized spectra at iteration $\mathbf{\textit{i}}$, while $\mathbf{\textit{P}_\textit{i}}$ represents the estimated design parameters at the corresponding iteration.
% % In determining the dimensionality of $\mathbf{\hat{\textit P}}$, the methodology involves evaluating the distance, measured using a loss function, between $\mathbf{\textit{S}_\textit{i}}$ and $\mathbf{\hat{\textit S}}$, rather than between $\mathbf{\textit{P}_\textit{i}}$ and $\mathbf{\hat{\textit P}}$. Subsequently, the procedure encompasses updating $\mathbf{\textit{P}_\textit{i}}$ in the direction that minimizes this distance during each iteration.
% % 
% % ----
% % 
% To simulate a real-world scenario where we have both the real device and its spectra, we first determine values for the ground truth, denoted as $\mathbf{\hat{\textit P}}$, and generate spectra $\mathbf{\hat{\textit S}}$ from a virtual structure defined by $\mathbf{\hat{\textit P}}$. The objective is to estimate $\mathbf{\hat{\textit P}}$ using $\mathbf{\hat{\textit S}}$, as direct measurement of $\mathbf{\hat{\textit P}}$ is not feasible. 
% To achieve this, we initially create a virtual structure with limited prior knowledge provided by domain experts, and we randomly draw the initial parameters $\mathbf{\textit{P}_\textit{0}}$ from a suitable distribution. Subsequently, we generate $\mathbf{\textit{S}_\textit{0}}$ from $\mathbf{\textit{P}_\textit{0}}$.
% We then employ a distance metric to quantify the discrepancy between the estimated and ground truth parameters. 
% The process involves obtaining a loss value followed by backpropagation, which provides guidance on whether the elements of $\mathbf{\textit{P}_\textit{0}}$ should be adjusted upwards or downwards. This iterative process can be generalized using $\mathbf{\textit{P}_\textit{i}}$ and $\mathbf{\textit{S}_\textit{i}}$, where $\textit{i}$ denotes the iteration number.
% As we keep iterating, $\mathbf{\textit{S}_\textit{i}}$ approaches $\mathbf{\hat{\textit S}}$ and presumably $\mathbf{\textit{P}_\textit{i}}$ approaches $\mathbf{\hat{\textit P}}$, where $\mathbf{\hat{\textit P}}$ is the parameter set we aim to find.
% \subsubsection{Physics: spectrum fitting}

% \textbf{Parallelization}
% This means that getting a spectrum for a single structure needs RCWA to be repeated as many as the number of wavelength in use. This is where paralleilzation comes in handy.
% % \textbf{Spectrum generation with parallelization}
% JAX support PMAP function which parallelize the loop. We can utilize this to perform RCWA simulation with the same condition but different wavelength to get spectrum.
% Other way is to use Ray.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{sections/applications/images/pmap.png}
%     \caption{Performance test: calculation time by FTO sweep. The result is normalized by NumPy case from the same options to compare the behavior of other backends. In these plots, black dashed line is $y=1$ and the results of NumPy cases lie on this line since they are normalized by themselves.}
%     \label{fig:benchmark/backend}
% \end{figure}

% \textbf{SETUP}
%% original
% We demo here a exemplary case that has 6 design parameters to estimate. Using spectrum fitting, we will evaluate 6 different gradient based algorithms, namely momentum, Adagrad, RMSProp, Adam, RAdam and NAdam.
% This test is designed to see the behavior of each algorithms from the same starting points. To mitigate the effect of starting value, it was repeated 10 times. 
% 
% Here, we present an exemplary case involving the estimation of six design parameters. 
% Employing spectrum fitting, we evaluate six distinct gradient-based algorithms: momentum, Adagrad, RMSProp, Adam, RAdam, and NAdam.
% As this test aims to observe and compare the behavior of each algorithm, all algorithms start from identical initial points and undergo 100 iterations. 
% This set is repeated 10 times, with each repetition having different initial points to mitigate the randomness of initial points selection, which play crucial role in local optimization algorithms. 

Here, we introduce an exemplary case concerning the estimation of six design parameters \cyp{as discussed in} \ref{sec:ocd}. Employing spectrum fitting, we evaluate six distinct gradient-based algorithms: Momentum, Adagrad \cite{duchi2011adaptive-adagrad}, RMSProp \cite{hinton2012neural-rmsprop}, Adam \cite{DBLP:journals/corr/KingmaB14} and RAdam \cite{liu2019radam}.

The objective of this test is to observe and compare the behavior of each algorithm. To ensure consistency, all algorithms begin from identical initial points and undergo 100 iterations. Furthermore, this process is repeated 10 times, with each repetition involving different initial points. This approach is adopted to mitigate the randomness associated with initial point selection, a factor that plays a crucial role in local optimization algorithms.

\begin{figure}[ht]
    \centering        \includegraphics[width=\textwidth, trim=8 8 8 8,clip]{sections/applications/images/ocd-optimize.png}
    \caption{\textbf{Loss Curves of Various Gradient-Based Algorithms for Spectrum Fitting.}
    This figure illustrates the loss curves of different gradient-based algorithms for spectrum fitting. Each algorithm undergoes 100 iterations. The Y-axis represents the distance, while the X-axis indicates the number of iterations. Across all algorithms, 10 tests are conducted with different starting points, which are shared. Lines of the same color denote shared initial values among the plots.}
    \label{fig:ocd-optimize}
\end{figure}

% \textbf{RESULT}
%% original
% Fig. \ref{fig:ocd-optimize} shows the optimization performance. 
% Within these data, we can see that Adagrad and RMSprop have faster loss decline at the beginning but later it is slightly saturated and converged to relatively higher region.
% Adam and RAdam, they shows comparable final place but the bandwidth of the curves is different. RAdam shows narrower one and this seems helpful to decrease the number of initial conditions. but who knows?

% Optimization algorithm itself is beyond of this work. We will stop here.

Observing the optimization performance depicted in Fig. \ref{fig:ocd-optimize}, it is notable that Adagrad and RMSprop exhibit a more rapid initial decline in loss. However, as the process progresses, the slope of the curves diminishes, and they converge to a relatively higher value (7E-5).

The Adam-family algorithms, namely Adam and RAdam, exhibit similarities in the early stages of optimization across the 10 repetitions. 
However, NAdam struggles to overcome local minima, whereas both Adam and RAdam reach a loss value of 1E-6. Furthermore, these two algorithms maintain the initial slope of the curve during iterations, indicating that better fitting can be expected by increasing the number of iterations. Adam achieves the best result overall, but RAdam demonstrates a more consistent performance across different cases, suggesting better robustness.

% It is essential to acknowledge that the optimization algorithm itself falls beyond the scope of this study, thus concluding our analysis at this point.

% In this manner, a new algo or hypotheses can be evaluated.

-----------------

% \paragraph{Limitation}
% Hyperparameter tuning is not enough.

\textbf{Advanced topics, Further work, optional}
These are beyond of this paper

In future works, We plan to investigate these research topics.

a) development of new optimization method helped by physical model
b) investigate any hypothesis on relation between number of iteration and number of episode - sweetspot.
c) correlation between finding S and finding P.

a) OCD is a field that has foundational model based on physics. 

b) as shown, initial point has big impact. 

c) The purpose of OCD is to find the parameters so we presume that smaller distance in S is connected to more correct parameters P. This is not always true, though.

% \textbf{Sweetspot}

% As the number of parameters increases, we encounter the curse of dimensionality and the local optima. We will approach in 2 ways: initial value sampling and optimization algorithms. Initial value can be chosen with many distribution such as normal or uniform. The range is a prior knowledge. Optimization algorithm decides the direction and the step size of update. This can help the problem to escape from local minima. We will evaluate GA, SGD, Adagrad, Adam and AdamW.


% \subsubsection{ML: Surrogate solver}
% \begin{wrapfigure}{r}{0.5\textwidth}
%     \includegraphics[width=0.9\linewidth]{sections/applications/images/ocd_ml_training.png}
%     \caption{Pd}
%     \label{fig:benchmark/backend}
% \end{wrapfigure}
% Even though this is very small time consuming compared to FDTD and FEM, but still suffers from big computation time. This is critical in mass production hence we need ML method to avoid this. We will suggest some ML models to approximate the physics in RCWA.

% The same model is used to make data that the size is 10k. 6k was used for training, 2k for validation and 2k for the test. The architecture has 3 layers, and each has 100 neurons.
% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=0.5\textwidth]{sections/applications/metasurface/images/ocd_ml_training.png}
% %     \caption{Performance test: calculation time by FTO sweep. The result is normalized by NumPy case from the same options to compare the behavior of other backends. In these plots, black dashed line is $y=1$ and the results of NumPy cases lie on this line since they are normalized by themselves.}
% %     \label{fig:benchmark/backend}
% % \end{figure}

% Figure shows the result. As epoch goes, the loss of validation set decreases and saturated at 1E-5. The time took only 0.1\% of physics based solution. This is applicable where the domain is confined: HVM (high volume manufacturing) is a good scenario since each process step has very tight control window which means the data distribution can be found in early stage. 

==> sections/background/background.tex <==
\subsection{Electromagnetic simulation using RCWA}
\label{sec:rcwa}
\input{sections/meent_framework/rcwa}
\subsection{Application of RCWA}
\begin{figure}
    \centering        
    \includegraphics[width=.6\linewidth, trim=2 8 8 8,clip]{sections/background/images/image.png}
    \caption{Applications of RCWA. (a) is one dimensional beam deflector using metasurface. (b) is OCD process.} 
    \label{fig:modeling-representation}
\end{figure}
\paragraph{Electromagnetic metasurface}
A metasurface is a two-dimensional, artificially designed device capable of controlling light, specifically electromagnetic waves, with a thickness smaller than the wavelength of use \cite{kildishev2013planar-metasurface, yu2014flat-metasurface, sun2019electromagnetic-metasurface}. This unique feature enables the creation of devices that were previously unattainable with naturally occurring materials.
An example of metasurface application is depicted in Figure \ref{aa}, showing a beam deflector.
% However, due to its complex and often unpredictable nature, designing a metasurface requires extensive simulations to determine the optimal design parameters that meet the desired specifications. RCWA serves as a valuable tool for evaluating the performance of intermediate device structures during the design process.
\paragraph{Optical critical dimension metrology}
RCWA finds one of its most successful industrial applications in optical metrology within the semiconductor fabrication. It serves to estimate the dimensions of device structures between process steps, thereby effectively monitoring excursions and maximizing yield due to its non-destructive nature and high throughput capabilities.
As illustrated in Figure \ref{fig:ocd-scheme}, light with multiple wavelengths is directed onto the surface of the sample, and the reflected light is collected by a detector. This reflected light is then decomposed by wavelength, and the intensity of each wavelength is recorded. This spectral data is utilized to estimate the structure of the sample.

==> sections/checklist/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We believe that the contents and the scope of our paper, closely reflect the claims in abstract and introduction sections.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
    %     \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
    %     \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
    %     \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    % \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The conclusion in Section \ref{sec:limitations} includes a discussion about the limitations of our work.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
    %     \item The authors are encouraged to create a separate "Limitations" section in their paper.
    %     \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
    %     \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
    %     \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
    %     \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
    %     \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
    %     \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    % \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper is more related to empirical results.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include theoretical results. 
    %     \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
    %     \item All assumptions should be clearly stated or referenced in the statement of any theorems.
    %     \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
    %     \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
    %     \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    % \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code for reproducing presented experiments will be fully provided in our GitHub repository at \href{https://github.com/kc-ml2/meent}{https://github.com/kc-ml2/meent}.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
    %     \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
    %     \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
    %     \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
    %     \begin{enumerate}
    %         \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
    %         \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
    %         \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
    %         \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
    %     \end{enumerate}
    % \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main simulator code and tutorial code are provided in our GitHub repository at \href{https://github.com/kc-ml2/meent}{https://github.com/kc-ml2/meent}. The code for generating experimental data will also be made available. Also additional contents will be provided in supplementary if necessary.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that paper does not include experiments requiring code.
    %     \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
    %     \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
    %     \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
    %     \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
    %     \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    % \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The details of each experiment are described in Appendix \ref{appendix:pde-training}, \ref{appendix:meta-training} and \ref{appendix:ocd_demonstration}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
    %     \item The full details can be provided either with the code, in appendix, or as supplemental material.
    % \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    The statistics of our experiments through Sections \ref{sec:fno}, \ref{sec:mbrl} and \ref{sec:ocd}, have taken considerations as follows:

    Test result and the train/test split of Section \ref{sec:fno} are summarized in Appendix \ref{appendix:pde-error} and \ref{appendix:pde-training}. Statistics for nine different physical conditions are reported. We do not think that testing each condition against multiple random seeds have significant impact on the results, due to the deterministic nature of the models.
    
    Training curve of Section \ref{sec:mbrl} summarized in Figure \ref{fig:meta-curve} was generated with three randoms seeds, which we believe suffice to test robustness of stochastic parts of the models. Additionally, since our environment is deterministic, historical maximum values are focused rather than usual "evaluation rewards" presented in reinforcement learning papers.
    
    For Section \ref{sec:ocd}, Figure \ref{fig:ocd-optimize} displays 10 repeated results using lines instead of error bars, owing to its logarithmic scale.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
    %     \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
    %     \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
    %     \item The assumptions made should be given (e.g., Normally distributed errors).
    %     \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
    %     \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
    %     \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
    %     \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    % \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Detailed resource specifications for benchmark and experiment, etc are provided in Appendix \ref{appendix:benchmarks}, Appendix \ref{appendix:meta-training} and Appendix \ref{appendix:pde-training}.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
    %     \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
    %     \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    % \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have read through code of ethics and conform that our research does not violate them.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
    %     \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
    %     \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    % \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work is based on physics simulation that is hard to make direct societal impacts.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that there is no societal impact of the work performed.
    %     \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
    %     \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
    %     \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
    %     \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
    %     \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    % \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our electromagnetic simulator hardly have relation to the risks.
    % Section \ref{appendix:benchmark-fourier_series_implementations} explains the importance of hyperparameter.
    % \item[] Guidelines: 
    % \begin{itemize}
    %     \item The answer NA means that the paper poses no such risks.
    %     \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
    %     \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
    %     \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    % \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, license are clearly stated in Appendix \ref{appendix:licenses} and will be credited in acknowledgement section.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not use existing assets.
    %     \item The authors should cite the original paper that produced the code package or dataset.
    %     \item The authors should state which version of the asset is used and, if possible, include a URL.
    %     \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
    %     \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
    %     \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
    %     \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
    %     \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    % \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Detailed explanations are provided in Appendix \ref{appendix:background_theory}, \ref{appendix:program_sequence}, \ref{appendix:benchmarks} and \ref{appendix:applications}.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not release new assets.
    %     \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
    %     \item The paper should discuss whether and how consent was obtained from people whose asset is used.
    %     \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    % \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no existence of instructions, since no human subjects are employed.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
    %     \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    % \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We believe there are no potiential risks, since no human subjects are employed.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
    %     \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
    %     \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    % \end{itemize}

\end{enumerate}

==> sections/introduction/bin/introduction_old.tex <==
Harnessing light-matter interaction to design a device with sub-wavelength scale structure has a wide range of applications, including high-efficiency solar cells \cite{peter2019nanostructures, snaith2013perovskites}, semiconductor design and manufacture \cite{zayats2013active, chang1992arrayed}, ultra-thin metalenses and displays \cite{zhang2018ultra, aieta2012aberration}, optical computation \cite{fang2005sub, silva2014performing}, and so on. Their implication to the real world is far-reaching, from better renewable energy production to enhanced user experience to next-generation computation.

But designing such nanophotonic devices is a challenging problem, which often boils down to a combinatorial optimization problem \cite{wang2023scientific}: the size of the design space of such a device, which can easily go over $10^{80}$ \cite{park2024sample}, is too large to explore the entirety of it in a brute-force manner. In addition, assessing a single data point in the design space is time-consuming due to the nature of electromagnetic simulation that requires precise calculations of interference and diffraction of electromagnetic wave, whose runtime ranges up to days per a single candidate structure \cite{burger2008benchmark}.

Machine learning (ML) is a promising candidate to solve such a problem, and with the advent of deep learning, optics community has been made successful efforts to leverage modern machine learning techniques to find both better optimization algorithms and faster electromagnetic simulators \cite{malkiel2018plasmonic,melati2019mapping,jiang2019global}.
Deep generative model \cite{so2019designing} was used to reduce computational cost compared to traditional optimization algorithm. 
The feasibility of using reinforcement learning (RL) to design nanophotonic devices were showed in \cite{seo2021structural}. 
Back-propagation, utilizing automatic differentiation (AD), has been employed in \cite{colburn2021inverse, grcwa, kim2023torcwa} to find design parameters of nanophotonic structures .
Furthermore, physics-informed neural networks \cite{raissi2019physics}, neural operators \cite{li2020fourier}, and DeepONet \cite{lu2021learning} are being explored for their potential as surrogate electromagnetic simulators. These models aim to substitute heavy computational simulations with deep models that offer reduced computational load and increased robustness to hidden noise. 
% Additionally, super-resolution, a computer vision-driven ML technique, has found application in wafer metrology \cite{}. 
These researches show  significant potential of ML for uncovering new insights and expediting scientific discoveries.

On the other hand, from the viewpoint of ML, designing nanophotonic devices is an ideal environment for developing new ML algorithms, as they provide both ample simulation data to train ML models and well-defined optimization goals, often called figure of merit (FoM), for the real world applications. 
However, the integration of ML into computational nanophotonic physics presents unique challenges. Traditional EM simulation softwares, often written in languages like C or MATLAB, are not easily compatible with ML frameworks, which are predominantly developed in Python. 
Furthermore, the scarcity of public data in certain domains such as semiconductor optics, compounded by stringent intellectual property regulations, presents a formidable obstacle to ML researchers who does not have much domain expertise. 
Overcoming these barriers requires innovative approaches to data generation and sharing in order to enable ML researchers to explore new frontiers in computational physics.

In response to these challenges, we introduce \texttt{meent}, a Python-native EM simulation data generator designed to facilitate collaboration between ML and optics researchers. By providing ability to generate datasets that can be tailored to specific research needs, \texttt{meent} aims to democratize access to EM simulation data and accelerate scientific discovery in computational optics. Through empirical demonstrations, we illustrate the efficacy of \texttt{meent} as a powerful tool for tackling certain challenges in developing ML algorithms and advancing research in optics and related fields.

One of the key features of \texttt{meent} is its automatic differentiation (AD) \cite{baydin2018automatic} compatibility in modeling and optimization of nanophotonic devices in a continuous space. 
AD compatibility in ML toolchain is crucial \cite{moses2020instead, baydin2018automatic}, and while some existing tools support vector modeling and others support automatic differentiation, none offer both functionalities simultaneously. 

Another notable feature of \texttt{meent} is that, for developer ergonomics, \texttt{meent} is developed to be compatible with three different backend frameworks: NumPy \cite{harris2020array}, JAX \cite{jax2018github}, and PyTorch \cite{paszke2019pytorch}. This flexibility is crucial as many researchers can benefit from a deep understanding of a single framework rather than being a generalist of multiple tools. Moreover, transitioning between frameworks can be a non-trivial task, especially for scientific simulators requiring domain-specific knowledge. By supporting multiple backends, \texttt{meent} facilitates easy and swift adoption, accommodating researchers with varying levels of expertise and preferences. 

Our key contributions can be summarized as follows:
\begin{itemize}
    \setlength\itemsep{0em}
    \item \ant{maybe simplify some sentences from intro to here 1} (meent)
    \item \ant{maybe simplify some sentences from intro to here 2} (meent supports intersection of other EM simulators, making meent unique, versatile)
    \item \ant{weaker word. Novel} Provide one simple baseline and one state-of-the-art baseline for each downstream metasurface tasks.
    \item OCD metrology that highlights meent's strong features.
\end{itemize}


%% original
% As the era of machine learning begins, everyone has tried to find a way to adopt ML to maximize the benefits. Optics researchers as well started to apply ML techniques to their research and proved its usefulness. 
% RL was used for inverse problem in metasurface design \cite{}, optimizers were introduced (??) \cite{}, and computer vision driven ML techniques were used in wafer metrology \cite{}.
% Back-propagation (using automatic differentiation, AD) was equipped to calculate the gradient of figure of merit with respect to the design parameters \cite{}. More than being an assistant of physics, there have been efforts to replace EM simulation with ML models as universal approximators \cite{}. They are used in metrology, and scientific ML such as PINN and Neural operator is intensively investigated in many teams.



%% original
% Other than the algorithms mentioned above, the development of infrastructure for ML also strongly affected computational physics. One of the sources that incurred ML skyrocketing is the explosive increase of computational capability. EM simulation is calculation hungry as is ML.
% 
% As is ML, EM simulation is calculation hungry which is a bottleneck for applications. To relieve, we can intuitively think of two approaches: make simulation model smaller or have more power. If we find answers from ML perspective, the former is using an artificial neural network (ANN) as a surrogate model and the latter is utilizing the infra driven by ML industry.

%\st{Beyond the algorithms, the advancement of ML infrastructure has significantly impacted computational physics. The explosive growth in computational capabilities has been a significant catalyst for the proliferation of ML. This surge in computational power has facilitated the flourishing of ML, a field that typically requires considerable computational resources. Given this context, it is rational to extend this advancement to the domain of computational physics, which operates within a calculation-intensive regime similar to ML. Frameworks for big data processing, such as Spark and Ray, provide methods for parallelized and distributed computing, thereby enabling researchers to squeeze computational resources without requiring in-depth knowledge of infrastructure engineering.}

% Additionally, tools like JAX, with its pmap function, offer simpler parallelization, thereby enabling researchers to leverage computational resources without requiring in-depth knowledge of infrastructure engineering.

% ---
%% original
% A surrogate model using ANN is widely investigated one in scientific machine learning (SciML) society. PINN, NO are examples. FNO showed good performance.
% 
% A framework for big data such as Spark and Ray, provides methods for parallelized and distributed computing. Smaller but easier is provided by JAX with the function pmap. These helps researchers to utilize facilities without understanding and engineering the infrastructure.

% Surrogate models using ANNs are widely explored within the scientific machine learning (SciML) community, with examples including PINN and Neural Operators, which have demonstrated promising performance.
% Frameworks for big data processing, such as Spark and Ray, provide methods for parallelized and distributed computing. Additionally, tools like JAX, with its pmap function, offer simpler parallelization, thereby enabling researchers to leverage computational resources without requiring in-depth knowledge of infrastructure engineering.

% In short, ML-related technologies can be a breakthrough for computational physics, and to make it happen, Python-written simulation engine is a must.

% Because computational physics deal with classical theories in long history, the code exists in mature programming languages such as C family or MATLAB. But as we know, ML community is mainly driven by Python. This has been a rising star that has low hurdle to enter, with the cost of computing capability loss, though. But it's absolutely affordable considering the time for preparation of experiment especially in R\&D stage. This enabled many optics researchers to apply ML in much fast speed and make result.

% For such a reason, we have developed Meent, a Python-native data generator, to invite ML researchers to optics. 

% As many fields of research suffer from lack of data, optics, especially semiconductor related, also does because of the cost for data: manufacturing chip isn't cheap at all, and the data made from semiconductor fabrication plant is strictly prohibited due to intellectual property. 
% This hinders ML researchers to dive in this field, and optics researchers to apply the latest ML techniques to their work.
% Meent is here to help. By providing data which can be manually designed anytime, ML techniques can be evaluated and the hypotheses are verified with the data.

% We will demonstrate its value as a data generator by solving ML problems with good techniques.

% ----
% Analogous to ML, electromagnetic (EM) simulation requires substantial computational resources, thus posing a bottleneck for applications. To address this challenge, two intuitive approaches can be explored: reducing the complexity of simulation models or enhancing computational power. From an ML standpoint, the former entails the utilization of artificial neural networks (ANNs) as surrogate models, while the latter leverages the advanced infrastructure of ML.

% --

% OCD side benefit
% Analogous to ML, electromagnetic (EM) simulation requires substantial computational resources, thus posing a bottleneck for applications. To address this challenge, two intuitive approaches can be explored: reducing the complexity of simulation models or enhancing computational power. 

% These can be tackled by ML technologies: the former entails the utilization of artificial neural networks (ANNs) as surrogate models, while the latter leverages the advanced infrastructure of ML.

% Bottom line is, ML-related technologies can be a breakthrough for computational physics, and to make it happen, a Python-written simulation engine is a must.
% -----

% In short, ML-related technologies can be a breakthrough for computational physics, and to make it happen, a Python-written simulation engine is a must.

%As we have observed thus far, it becomes evident that the relationship between ML and computational physics is mutually beneficial. From the perspective of physics, ML holds substantial promise for revolutionizing computational physics by offering novel solutions to enduring challenges. Similarly, from the standpoint of ML, computational physics provides an ideal environment for hypothesis testing, benefitting from access to unlimited simulation data that can be tailored to meet specific experimental conditions.
%At the heart of this collaboration lies the adoption of ML methodologies, which leverage their robust computational capabilities to enhance traditional approaches in computational physics. This synergy holds significant potential for uncovering new insights and expediting scientific discoveries.



% Machine learning (ML) has emerged as a transformative force across numerous domains, including computational physics. 
% Its potential to revolutionize this field is profound, offering innovative solutions to longstanding challenges. 
% Central to this transformation is the adoption of ML methodologies, which harness vast computational capabilities to enhance traditional approaches in computational physics. 
% This synergy between ML and computational physics holds promise for unlocking new insights and accelerating scientific discovery.


% Machine learning (ML) has emerged as a transformative force across numerous domains, including computational physics. Its potential to revolutionize this field is profound, offering innovative solutions to longstanding challenges. Central to this transformation is the adoption of ML methodologies, which harness vast computational capabilities to enhance traditional approaches in computational physics. This synergy between ML and computational physics holds promise for unlocking new insights and accelerating scientific discovery.

%--

% Because computational physics deals with classical theories that have a long history, the code often exists in mature programming languages such as the C family or MATLAB. However, as we know, the ML community is primarily driven by Python. While Python may entail some loss in computing capability, it offers a low barrier to entry. This trade-off is acceptable, especially considering the time required for experiment preparation, particularly in the R\&D stage. This accessibility has enabled many optics researchers to apply ML more rapidly and achieve results.

%However, despite its transformative potential, the integration of ML into computational physics poses unique challenges. Traditional computational physics codes, often written in mature languages like the C family or MATLAB, may not readily accommodate ML methodologies, which are primarily developed in or for Python. This discrepancy necessitates a concerted effort to bridge the gap between these disparate programming paradigms while capitalizing on the strengths of each.

%--

% For this reason, we have developed Meent, a Python-native data generator, to attract ML researchers to optics.

% Many fields of research suffer from a lack of data, and optics, especially semiconductor-related studies, are no exception. The high cost of data acquisition, as manufacturing chips is expensive, coupled with strict intellectual property regulations governing data from semiconductor fabrication plants, hinders ML researchers from delving into this field. Simultaneously, it restricts optics researchers from applying the latest ML techniques to their work. Meent aims to alleviate these challenges by providing data that can be manually designed at any time, enabling ML techniques to be evaluated and hypotheses to be verified using this data.

%Furthermore, the scarcity of data in certain domains, such as optics and semiconductor-related studies, presents a formidable obstacle to ML researchers seeking to apply their techniques. The prohibitive costs associated with data acquisition, compounded by stringent intellectual property regulations, hinder progress in these fields. Overcoming these barriers requires innovative approaches to data generation and sharing, enabling ML researchers to explore new frontiers in computational physics.

% --

% We will demonstrate the value of Meent as a data generator by solving ML problems with proven techniques.



% ----

% Machine learning (ML) has emerged as a transformative force across numerous domains, including computational physics. Its potential to revolutionize this field is profound, offering innovative solutions to longstanding challenges. Central to this transformation is the adoption of ML methodologies, which harness vast computational capabilities to enhance traditional approaches in computational physics. This synergy between ML and computational physics holds promise for unlocking new insights and accelerating scientific discovery.

% However, despite its transformative potential, the integration of ML into computational physics poses unique challenges. Traditional computational physics codes, often written in mature languages like the C family or MATLAB, may not readily accommodate ML methodologies, which are primarily developed in Python. This discrepancy necessitates a concerted effort to bridge the gap between these disparate programming paradigms while capitalizing on the strengths of each.

% Furthermore, the scarcity of data in certain domains, such as optics and semiconductor-related studies, presents a formidable obstacle to ML researchers seeking to apply their techniques. The prohibitive costs associated with data acquisition, compounded by stringent intellectual property regulations, hinder progress in these fields. Overcoming these barriers requires innovative approaches to data generation and sharing, enabling ML researchers to explore new frontiers in computational physics.

% In response to these challenges, we introduce Meent, a Python-native data generator designed to facilitate collaboration between ML and optics researchers. By providing access to curated datasets that can be tailored to specific research needs, Meent aims to democratize access to data and accelerate scientific discovery in computational physics. Through empirical demonstrations, we illustrate the efficacy of Meent as a powerful tool for solving ML problems and advancing research in optics and related fields.

% -----

% In summary, ML-related technologies have the potential to revolutionize computational physics. Python-written simulation engines are crucial in this context, as Python's accessibility has facilitated rapid adoption among ML researchers, albeit with some compromises in computational capability. Meent, a Python-native data generator, has been developed to bridge the gap between ML and optics research. By providing easily accessible data generation capabilities, Meent facilitates the evaluation of ML techniques and the validation of hypotheses in optics research. Its value as a data generator will be demonstrated through the application of advanced ML techniques to solve various problems.



% metasurface is an field of research that investigates the principles and applications of nano-scale photonic devices showing unexpected behaviors. This unpredictability naturally requires tons of simulations to find design parameters that maximize or minimize some characteristics of interest.
% Industry, RCWA is highly used for optical metrology in semiconductor manufacturing, called Optical Critical Dimension (OCD) metrology. This aims to find design parameters of the device structures in real world by spectrum fitting. 

% \textcolor{blue}{
% We picked RCWA since it's vastly used technique in both academy and industry thanks to its critically high throughput under some conditions. In academia, metasurface is an interesting field of research that investigate the interaction between light and matter. This naturally leads to find design parameters that maximize or minimize some characteristics of interest. For this reason, non-profitable, there are few free SW which is small piece of codes dedicated to specific experiments rather than complete product hence remaining options is the major giant tech companies such as Ansys provides solutions with cost. Industry, RCWA is highly used for optical metrology in semiconductor manufacturing, called Optical Critical Dimension (OCD) metrology. This aims to find design parameters of the device structures in real world by spectrum fitting. SW is strongly chained to solution provider's HW hence not available for researchers outside organization.
% }


% \textcolor{red}{
% Optics, the study of light and the interaction of light and the matter, [has long history and important in sciecnce]. [some studies require numerical simulations] [some problems can't be solved with classical optics so ML methods adopted]
% }
% \textcolor{red}{[Maybe a lil bit of literature(lit.) of nanophotonics and photonics here(sub branch of optics). unexpected behavior when magnifies down to nano scale (such as high impact cell), also lit. of flat optics based on n layer metagratings. because our tasks of 1) surrogate solver 2) parallelization 2) MBRL all lies in this lit.
% ]}
    

% Compared to other electromagnetic solvers, such as the finite element method (FEM) or the finite-difference time-domain (FDTD) method, RCWA offers advantages in terms of non-iterative and deterministic characteristics which makes RCWA simple and fast hence a popular choice for industrial use.
% Representative applications of RCWA are Optical Critical Dimension metrology (OCD) and metasurfaces design.


% The primary goal of Meent is to accelerate ML research in the field of optics. To achieve this, we have developed Python-written packages, enabling seamless integration with the rich ecosystem of ML packages available within the Python community.

% By leveraging Python as the programming language, Meent eliminates the communication overhead that arises when interfacing between Python and MATLAB, the de-facto language for photonics applications. This seamless integration empowers researchers in the photonics to harness the full potential of well-developed ML tools and libraries within Python, facilitating faster and more efficient experimentation and analysis in their work. The introduction of Meent thus represents a significant advancement in the domain of photonics research and its integration with machine learning methodologies.



==> sections/introduction/introduction_diet.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth, trim=0 0 0 0,clip]{sections/introduction/figures/image4.png}
\caption{\textbf{Summary.} \textit{Simulation Algorithm} depicts the process flow of the electromagnetic simulation algorithm, RCWA, in Meent. \textit{Applications} present the most representative problems that Meent can be utilized for.}
\label{fig:meent-summary}
\end{figure}

% \ant{EM importance}
Harnessing light-matter interactions at the sub-wavelength scale has a wide range of applications, including high-efficiency solar cells \cite{peter2019nanostructures, snaith2013perovskites}, semiconductor design and manufacture \cite{zayats2013active, chang1992arrayed}, ultra-thin metalenses and displays \cite{zhang2018ultra, aieta2012aberration}, and optical computation \cite{fang2005sub, silva2014performing}. These advancements are profound, leading to improved renewable energy production, enhanced user experiences, and pioneering developments in next-generation computation.

Large portions of those applications naturally entail electromagnetic simulations for solving Maxwell's equation. Oftentimes, such simulations are time-consuming, due to the nature of them requiring precise calculations of interference and diffraction of electromagnetic wave. For example, assessing a single data point in the design space can take runtime extending up to days per candidate structure \cite{}. 

Assisted with physical simulators, machine learning (ML) is promising candidate to solve such a problem with the advent of deep learning. ML is being actively embraced across scientific domains to substitute heavy simulations with deep models that serve as surrogate solvers, offering increased robustness to hidden noise. Not to mention optics field, governing equations of physical systems from diverse domains have been successfully tackled by seminal works such as neural operator, a data-driven approach. The equations ranges from linear to nonlinear dynamics \cite{li2020fourier, cai2021deepm, li2020neural, li2023fourier, lu2021learning, lu2022comprehensive, jin2022mionet}, forward to inverse problems \cite{raissi2019physics}, and high-dimensional equations \cite{sirignano2018dgm}.
Also, the feasibility of reinforcement learning (RL) has been demonstrated in the magnetic control of tokamak plasmas \cite{degrave2022magnetic} and classical mechanics \cite{lillicrap2015continuous, todorov2012mujoco}, and inverse design of optical device \cite{seo2021structural} highlighting its potential in addressing complex optics systems. 

The data-intensive nature of ML necessitates the development of efficient, easily accessible and compatible solutions.
% further complicates the scenario, 
% seminal works such as neural operators, a data-driven approach.
% of partial differential equations, 
However, traditional EM simulation software are often written in languages like C or MATLAB, presenting compatibility challenges with ML frameworks in conjunction with automatic differentiation (AD), which predominantly use Python. 
Moreover, the scarcity of publicly available data in semiconductor optics, coupled with stringent intellectual property regulations, poses significant obstacles for ML researchers lacking domain expertise. 
Overcoming these barriers requires innovative approaches to data generation and sharing in order to enable ML researchers to explore new frontiers in computational optics.

In response to these challenges, we introduce \texttt{meent}, a Python-native differentiable EM simulator based on Rigorous coupled-wave analysis (RCWA).

RCWA \cite{Moharam:81, Moharam:95-formulation, Moharam:95-implementation, Lalanne:96, Granet:96, Li:96, rumpf-dissertation, Li:hal-00985928} is a prominent electromagnetic (EM) simulation algorithm for interpreting light-matter interactions by solving Maxwell's equations. RCWA's high throughput and deterministic nature have led to its widespread adoption in optics across academia and industries, demonstrating efficacy in various applications.

Key features of \texttt{meent} include its compatibility with automatic differentiation (AD) \cite{baydin2018automatic, moses2020instead} for modeling and optimizing nanophotonic devices in a continuous space. 
AD compatibility in ML toolchain is pivotal, and while some existing tools support vector modeling and others support AD, none offer both functionalities simultaneously. 
For developer ergonomics, \texttt{meent} is developed to be compatible with three different backend frameworks: NumPy \cite{harris2020array}, JAX \cite{jax2018github}, and PyTorch \cite{paszke2019pytorch}. This flexibility is crucial as many researchers can benefit from a deep understanding of a single framework rather than being a generalist of multiple tools. 
Moreover, transitioning between frameworks can be a non-trivial task, especially for scientific simulators requiring domain-specific knowledge. 
By supporting multiple backends, \texttt{meent} facilitates easy and swift adoption, accommodating researchers with varying levels of expertise and preferences. 

% \ant{applications of RCWA, broad subject/our case study}
Utilizing \texttt{meent}, we provide case studies which include analyzing and designing metasurface---
% two-dimensional, 
an artificially designed nanophotonic device with a thickness smaller than the wavelength of light. When carefully designed, metasurface can achieve unprecedented control of light \cite{kildishev2013planar-metasurface, yu2014flat-metasurface, sun2019electromagnetic-metasurface}. 
 
Also, optical metrology, one of the most successful industrial applications within the semiconductor fabrication, is elucidated. Optical metrology serves to estimate the dimensions of device structures between process steps, thereby effectively monitoring excursions and maximizing yield due to its non-destructive nature and high throughput capabilities.

By providing the ability to generate datasets tailored to specific research needs and fruitful example applications, \texttt{meent} facilitates collaboration between ML and optics researchers, democratizing the access to EM simulation data, in a hope to accelerate scientific discovery in computational optics.
In a nutshell, our contributions are summarized as follows:
\begin{itemize}
\setlength\itemsep{0em}
\item Python-native electromagnetic simulation software supporting automatic differentiation and continuous space operation in ML frameworks under MIT license.
\item Demonstration of \texttt{meent}'s unique intersection with other EM simulators, enhancing its versatility.
\item Provision of baseline and state-of-the-art examples for downstream metasurface tasks.
\item Instructions(guideline?) for \texttt{meent}'s application in optical metrology, showcasing its unique features.

\item Development of \texttt{meent}, Python-native electromagnetic simulation code supporting automatic differentiation and continuous space operation in ML frameworks under MIT license.
% \item Provision of baseline and state-of-the-art examples for downstream metasurface tasks.
\item Demonstration of \texttt{meent}'s versatility with
% metasurface design 
exemplary cases where 
% baseline and state-of-the-art models are evaluated.
ML techniques are employed and evaluated.
% \item Highlighting \texttt{meent}'s application in OCD metrology, showcasing its robust features.
\item Providing manual having detailed explanations and instructions.

\end{itemize}

% \cyp{add many more references regarding optimizing optical structure using ML, by surveying PIRL paper's references, augenstein2023neural, etc.}

% \cyp{cite Meep and https://nips.cc/virtual/2023/poster/73583, mention COMSOL. \cite{kim2024datasets, oskooi2010meep}}

==> sections/introduction/introduction_diet2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth, trim=0 0 0 0,clip]{sections/introduction/figures/image4.png}
    \caption{\textbf{Summary.} \textit{Simulation Algorithm} depicts the process flow of the electromagnetic simulation algorithm, RCWA, in Meent. \textit{Applications} present the most representative problems that Meent can be utilized for.}
    \label{fig:meent-summary}
\end{figure}


% EM 시뮬레이션 그 자체는 샘플에서 광학 데이터를 뽑아내는 거다. 이를 역으로 이용해서 구조를 찾는건 인버스 프로블럼, 옵티미제이션이며 다양한 애플리케이션이 있다.솔라셀 찾기, 반도체 디자인 앤 제작(?), 메타렌즈, 디스플레이, 광학 컴퓨테이션?. 
% 
% 이런 인버스프러블럼들은 시간이 많이 걸린다. 많은 시뮬레이션을 요구한다. 또한 광학 시뮬레이션은 한번 돌릴때 많이 걸린다. 이런 문제를 해결하기 위해 ml이 떠오르는 대안이다. 검증된 예시는 이런저런 것들이 있다.
% 
% 그런데 이걸 이루는데는 문제가 있는데 바로 연속공간에서 사용가능한 머신러닝 기반의 파이썬 코드가 없다는 것이다.
% 
% 우리는 민트를 개발했다. rcwa를 사용하고 ml framework를 지원하며 연속공간에서 정의된다.
% 
% 민트는 광학에 ml을 이용하기도 좋고 ml을 광학에 이용하기도 좋다.
% 광학 입장에서는 시뮬레이션 시간을 단축할 수 있고 ml의 첨단 기법을 도입할 수 있다는 장점이 있다. ml입장에서는 이론을 검증할 테스트셋을 확보할 수있다. 또한 sciml을 위한 귀중한 자원이다.
% 
% 이를 증명하기 위해 우리는 3개의 애플리케이션을 통해 증명한다.

% EM simulation is a process to predict optical phenomena from sample.

% This is conversely used to find the property of the sample from optical characteristics.
% Inverse problem, which find causal factor from observations. 

% \textbf{EM intro}
% Electromagnetic wave analysis
% has a wide range of applications, including high-efficiency solar cells \cite{peter2019nanostructures, snaith2013perovskites}, semiconductor design and manufacture \cite{zayats2013active, chang1992arrayed}, ultra-thin metalenses and displays \cite{zhang2018ultra, aieta2012aberration}, and optical computation \cite{fang2005sub, silva2014performing}. These advancements are profound, leading to improved renewable energy production, enhanced user experiences, and pioneering developments in next-generation computation.

\textbf{\textcolor{blue}{EM design intro}}
Harnessing light-matter interactions
% 
\textcolor{blue}{to find a desired structure}
% 
of sub-wavelength scale 
% 
has a wide range of applications, including high-efficiency solar cells \cite{peter2019nanostructures, snaith2013perovskites}, semiconductor design and manufacture \cite{zayats2013active, chang1992arrayed}, ultra-thin metalenses and displays \cite{zhang2018ultra, aieta2012aberration}, and optical computation \cite{fang2005sub, silva2014performing}. These advancements are profound, leading to improved renewable energy production, enhanced user experiences, and pioneering developments in next-generation computation.

\textbf{\textcolor{blue}{Difficulty}} These are mostly inverse problems. They find the structure (causal factor) from optical phenomena (observations or design goal). These inverse problems are difficult. It takes many iterations. And a simulation itself takes much time.

Assessing a single data point in the design space is time-consuming due to the precise calculations required in electromagnetic simulations, with runtime extending up to days per candidate structure\cite{burger2008benchmark}. 

\textbf{\textcolor{blue}{ML as solution}} as a solution, ML is arising.

In general, Machine learning (ML) is actively embraced across scientific domains 
to substitute heavy computational simulations with deep models that serves as efficient surrogate solver, and increased robustness to hidden noise. 
From solving partial differential equations (PDEs) to inverse problems, seminal works such as physics-informed neural networks (PINN) \cite{raissi2019physics} integrating physics knowledge into loss functions, data-driven approaches like neural operators \cite{li2020fourier, cai2021deepm} and DeepONet \cite{lu2021learning} solve diverse domains of PDEs for linear/non-linear dynamics.
Also, heavy computation for solving high dimensional PDE was addressed in \cite{sirignano2018dgm}.
Theses researches shows ML's significant potential for uncovering new insights and expediting scientific discoveries.


\textbf{\textcolor{blue}{Bottleneck to adopt ML in optics}}
\textcolor{blue}{But it needs ML native simulator code to bring these into optics.}
Traditional EM simulation software, often written in languages like C or MATLAB, lacks compatibility with ML frameworks, which predominantly target Python. 

Additionally, the scarcity of public data in domains like semiconductor optics, compounded by stringent intellectual property regulations, presents a significant obstacle for ML researchers lacking domain expertise.

\textbf{\textcolor{blue}{present meent}}
In response to these challenges, we introduce \texttt{meent}, a Python-native EM simulator depicted in Figure \ref{fig:meent-summary}. 
Key features of \texttt{meent} include its compatibility with automatic differentiation (AD) \cite{baydin2018automatic} for modeling and optimizing nanophotonic devices in a continuous space, crucial in the ML toolchain \cite{moses2020instead, baydin2018automatic}. Additionally, \texttt{meent} supports multiple backend frameworks: NumPy \cite{harris2020array}, JAX \cite{jax2018github}, and PyTorch \cite{paszke2019pytorch}, enhancing its accessibility and adoption among researchers with varying expertise levels.

\textbf{\textcolor{blue}{benefit for each of optics and ML}}
By providing the ability to generate datasets tailored to specific research needs, it facilitates collaboration between ML and optics researchers, democratizing the access to EM simulation data, in a hope to accelerate scientific discovery in computational optics.

\textbf{\textcolor{blue}{contributions}}
Our contributions are summarized as follows:
\begin{itemize}
% \setlength\itemsep{0em}
\item Development of \texttt{meent}, Python-native electromagnetic simulation code supporting automatic differentiation and continuous space operation in ML frameworks under MIT license.
% \item Provision of baseline and state-of-the-art examples for downstream metasurface tasks.
\item Demonstration of \texttt{meent}'s versatility with
% metasurface design 
exemplary cases where 
% baseline and state-of-the-art models are evaluated.
ML techniques are employed and evaluated.
% \item Highlighting \texttt{meent}'s application in OCD metrology, showcasing its robust features.
\item Providing manual having detailed explanations and instructions.
\end{itemize}








==> sections/manual/applications/1D_shape.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth, trim=4 4 4 4, clip]{sections/manual/applications/figures/1d_vector_optim.png}
    \caption{\textbf{Optimization result of the 1D beam reflector in continuous space.} (a) The schematic of the metasurface with TiO$_2$ rectangular building block (b) The learning curve of the metasurface. (c) The reflectivity spectrum of the initial (dashed) and the final (solid) structure. Maximum reflectivity of the structure is red-shifted towards 600 nm and is enhanced as a result of the optimization. }
    \label{fig:1d_shape_result}
\end{figure}

% Aside from its capability to perform topology optimization for freeform metasurface design, Meent can also optimize metasurfaces with primitive shapes, such as rectangles or ellipses. 
In this example, we focused on designing a metasurface with a TiO$_2$ rectangular block on top of a SiO$_2$ substrate to maximize its TM reflectivity at a wavelength of 600 nm by controlling the width ($w$) and the thickness ($t$) of the block in continuous space. The period was set to 1000 nm along the x and y directions, with the $w$ and $t$ as the design parameters, initialized at $w = 100$ nm and $t = 325$ nm, respectively.

Unlike the common parameter sweep approach that requires numerous forward simulations for each parameter sample, Meent utilized the gradient of the figure of merit as guidance to optimize the design variables. As a result, it reached the optimum solution in as few as 50 iterations (Figure \ref{fig:1d_shape_result}b). After 100 iterations of optimization, the reflectivity of the metasurface shifted to 600 nm and increased by 18\% to 75\%, with the optimized values of $w^* = 110.06$ nm and $t^* = 335.04$ nm (Figure \ref{fig:1d_shape_result}c).


==> sections/manual/applications/bin/application_thinFilm.tex <==
% As the first case, we demonstrate the transmission spectrum of a multilayer thin film structure as shown in Fig. \ref{fig:thinfilm}a. The in-plane wavevectors are conserved and the electromagnetic field distribution can be decomposed into only two plane waves with different propagation directions in the z-axis. Our goal is to inverse design the transmission spectrum of this structure using the gradients from AD.

In the first case, we present the transmission spectrum of a multilayer thin film structure, as depicted in Fig. \ref{fig:thinfilm}a. In this structure, the in-plane wavevectors are conserved, and the electromagnetic field distribution can be decomposed into just two plane waves with distinct propagation directions along the z-axis. The primary objective of this case is to achieve inverse design of the transmission spectrum for this particular structure utilizing the gradients obtained from Automatic Differentiation (AD).


\begin{figure}[h!] % picture
    \centering
    \includegraphics[scale=0.5]{images/thinFilm_schematic.png}
    \caption{(a) Schematic diagram of the thin film system. (b) Transmission spectra of the target spectrum and the transmission spectrum at epoch 1 and 100. Please change the figure as what the comment dictates (c) Plot showing the RMSE value between the target spectrum and the transmission spectrum from the structure at each epoch.}
\label{fig:thinfilm}

\end{figure}


In this case, we define the figure of merit as the root mean squared error (RMSE) difference between the target spectrum and the actual spectrum, as illustrated in Fig. \ref{fig:thinfilm}b. We employ the gradient obtained from Automatic Differentiation (AD) to update the geometry of the multilayer thin film structure and utilize the ADAM optimizer for the optimization process. After twenty epochs of optimization, the resulting spectrum achieves an RMSE value of 0.01, as demonstrated in Fig. \ref{fig:thinfilm}c.

% OCD 예제로는 회전된 사각형을 패턴으로 갖는 소자의 구조를 찾는 실험을 해보자. 실제 제작된 소자에서 나온 계측 스펙트럼 $S_{device}$이 있고 모델링을 통해 얻은 합성 스펙트럼 $S_{model}$이 있어 최적화 과정을 통해 $S_{model}$을 $S_{device}$에 fitting해서 실제 구조를 알 수 있다.



==> sections/manual/briefing/briefing.tex <==
This is a manual and guidebook of Meent. Meent is an open-source Python code for electromagnetic simulation using Rigorous Coupled Wave Analysis (RCWA), composed of three main parts: modeling, electromagnetic simulation and optimization. 
% Meent is a classical EM simulation software using RCWA in Python which makes Meent an easy and simple solution to use and modify per use. 

Modeling supports both the Raster and Vector modeling each of which has own advantages.
% The accuracy of Raster modeling can be enhanced by increasing sampling frequency which makes improves the resolution of Fourier series. Vector modeling enables fine drawing of complex but sparse geometry which is appropriate for Optical Critical Dimension metrology.
Electromagnetic simulation utilizes RCWA that solves Maxwell's equations in the Fourier space.
Optimization is an important application since Meent provides the gradient of the Figure of Merit with respect to each of all the design parameters with the help of automatic differentiation. 

Meent has been being developed targeting to both of AI and physics domain. 
It encourages physics researchers to adapt the latest ML techniques without need for developing the simulation and optimization code from scratch, and ML researchers to find applications to develop and verify their experience with minimal understanding of the domain knowledge.


\textbf{License} MIT License.

\textbf{Download}
% The code and related documents are available in github repository. Also possible to install with pip.
\begin{itemize}
    \item github: \href{https://github.com/kc-ml2/meent}{github.com/kc-ml2/meent}
    \item pip: \colorbox{lightgray}{\lstinline{pip install meent}}
\end{itemize}
% \usepackage[svgnames]{xcolor}

\textbf{Requirement} Python $\geq$ 3.10 with external packages.

\textbf{Citation} Will be updated.

% \textbf{Technical contact} yongha@kc-ml2.com

% \textbf{About us}
% % \begin{figure*}[ht]
% %     \centering
% %     \includegraphics[width=1\textwidth]{chapters/generality/figures/aboutus.png}
% %     % \caption{Caption}
% %     \label{fig:enter-label}
% % \end{figure*}

% {{jLAB, KAIST}: Our research generally aims to create photonic and electronic devices having useful and non-intuitive functionalities, by exploring the intersections of optics, solid state physics, and other fields of physics at the nanoscale.}

% {{KC ML2}: KC has grown on the basis of technological development and customer satisfaction in the semiconductor and display equipment industry. ML2(Machine Learning Lab) is an independent research organization within KC. ML2 focuses on doing academic researches to keep close relationships with other research entities and build in-house expertises.}


==> sections/manual/cover/cover.tex <==
% Frontmatter data; appears on title page
% \title{Technical Document \\Template}
% \usepackage{authblk}
\title{meent - electromagnetic simulation software}
\subtitle{Manual}

\title{Meent}
\subtitle{electromagnetic simulation software}


\version{0.9.9-0}

\softwarelogo{\includegraphics[width=8cm]{chapters/cover/figures/meent_logo.png}}

\teamlogo{\includegraphics[width=.8\textwidth]{chapters/cover/figures/team.png}}

% \teamlogo{
%     \begin{figure}
%         \centering
%         \begin{subfigure}{0.5\textwidth}
%             \centering
%             \includegraphics[width=.8\textwidth]{chapters/cover/figures/ml2.png}            
%         \end{subfigure}%
%         \begin{subfigure}{0.5\textwidth}
%             \centering
%             \includegraphics[width=.8\textwidth]{chapters/cover/figures/jlab.png}            
%         \end{subfigure}
%         \label{fig:enter-label}
%     \end{figure}
%     }

\coverletter{
    code: \href{https://github.com/kc-ml2/meent}{github.com/kc-ml2/meent} \\
    \vspace{5pt}
    manual link: \href{arXiv.2111.00393}{arXiv.xxxx.xxxx}}

\author{\centering{\textit{Yongha Kim, Sanmun Kim, Kevin Octavian, Doyoung Heo,\newline Anthony W. Jung, Chaejin Park, Jeongmin Shin, Sunghyun Nam, Chanhyung Park, Juho Park, Sangjun Han, Jinmyoung Lee, \newline Seolho Kim, Min Seok Jang, Chan Y. Park}}}
% \author{\textbf{Yongha Kim, Sanmun Kim, Kevin Octavian, Doyoung Heo, Anthony W. Jung, Chaejin Park, Jeongmin Shin, Chanhyung Park, Juho Park, Sangjun Han, Jinmyoung Lee, Seolho Kim, Min Seok Jang, Chan Y. Park}}

% \affil[1]{KC Machine Learning Lab, Republic of Korea}
% \affil[2]{KAIST, Republic of Korea}
% \affil[3]{Caltech, United States}

\makeatletter
\renewcommand\maketitle{
    \begin{titlepage}
    \centering
    \@logocmd\par
    {\huge\bfseries\@title\par}
    {\huge\@subtitle\par}
    \bigskip
    {\Large\@ver\par}
    \vfill
    {\Large\bfseries\@coverletter\par}
    \vspace{240pt}
    {\Large \textbf{Contributors}} \\
    \vspace{10pt}
    {\Large \@author\par}
    \vfill
    % \@date
    \@teamlogo\par
    \end{titlepage}
}
\makeatother


==> sections/manual/cover/cover_1.tex <==
% Frontmatter data; appears on title page
% \title{Technical Document \\Template}
\title{Meent: Electromagnetic simulation software}
% \renewcommand\subtitle{dd}
\subtitle{Manual}
\version{0.9.9.1}

\softwarelogo{\includegraphics[width=8cm]{chapters/cover/figures/meent_logo.png}}

\teamlogo{\includegraphics[width=\textwidth]{chapters/generality/figures/aboutus.png}}

\author[1]{Yongha Kim}
\author[2, 3]{Sanmun Kim}
\author[2]{Kevin Octavian}
\author[2]{Doyoung Heo}
\author[1]{Anthony W. Jung}
\author[1, 2]{Chaejin Park}
\author[2]{Jeongmin Shin}
\author[2]{Chanhyung Park}
\author[2]{Juho Park}
\author[2]{Sangjun Han}
\author[1]{Jinmyoung Lee}
\author[1]{Seolho Kim}
\author[2]{Min Seok Jang}
\author[1]{Chan Y. Park}

\affil[1]{KC Machine Learning Lab, Republic of Korea}
\affil[2]{KAIST, Republic of Korea}
\affil[3]{Caltech, United States}


% \maketitle


==> sections/manual/main.tex <==
% \documentclass{article}
% % \documentclass{ol-softwaremanual}

% \usepackage{listings}
% \usepackage{arxiv}
% % \usepackage[utf8]{inputenc} % allow utf-8 input
% % \usepackage[sort&compress,numbers]{natbib}
% % \bibliographystyle{unsrtnat}
% \usepackage[backend=biber, sorting=none, style=numeric-comp]{biblatex}
% % \usepackage[backend=biber]{biblatex}
% \bibliography{references.bib}
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage[bb=boondox]{mathalfa}
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{stmaryrd}
% \usepackage{graphicx}
% % \usepackage{natbib}
% \usepackage{doi}
% \usepackage{amsmath}
% % \usepackage{romannum}
% \usepackage{fontspec}
% \usepackage{color}
% \usepackage{multirow}

% % \usepackage{kotex}
% \pagenumbering{arabic}
% \usepackage[affil-it]{authblk}
% \usepackage{blindtext}

% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{dirtytalk}
% \usepackage{csquotes}
% % \usepackage{cite}
% % \usepackage{setspace} \doublespacing
% \usepackage{esvect}
% % \usepackage{humanist}
% % \usepackage[T1]{fontenc}
% \usepackage{nicematrix}
% \usepackage{wrapfig}
% \setcounter{MaxMatrixCols}{12}
% \definecolor{dkgreen}{rgb}{0,0.6,0}
% \definecolor{gray}{rgb}{0.5,0.5,0.5}
% \definecolor{mauve}{rgb}{0.58,0,0.82}

% \lstset{
%     frame=trBL,
%     language=Python,
%     aboveskip=3mm,
%     belowskip=3mm,
%     showstringspaces=false,
%     columns=flexible,
%     % basicstyle={\small\ttfamily},
%     basicstyle=\linespread{1}\selectfont,
%     numbers=left,
%     xleftmargin=1cm,
%     % framexleftmargin=1cm,
%     numberstyle=\tiny\color{gray},
%     keywordstyle=\color{blue},
%     commentstyle=\color{dkgreen},
%     stringstyle=\color{mauve},
%     stepnumber=1,
%     breaklines=true,
%     breakatwhitespace=true,
%     tabsize=4
% }
% \renewcommand{\lstlistingname}{Code}
% \renewcommand{\arraystretch}{1.2}

% \title{Meent: An electromagnetic simulation software}

% \author[1\dag]{Yongha Kim}
% \author[2, 3\dag]{Sanmun Kim}
% \author[2]{Kevin Octavian}
% \author[2]{Doyoung Heo}
% \author[1]{Anthony W. Jung}
% \author[1, 2]{Chaejin Park}
% \author[2]{Jeongmin Shin}
% \author[2]{Chanhyung Park}
% \author[2]{Juho Park}
% \author[2]{Sangjun Han}
% \author[1]{Jinmyoung Lee}
% \author[1]{Seolho Kim}
% \author[2*]{Min Seok Jang}
% \author[1*]{Chan Y. Park}

% \affil[1]{KC Machine Learning Lab, Seoul 06181, Republic of Korea}
% \affil[2]{School of Electrical Engineering, KAIST, Daejeon 34141, Republic of Korea}
% \affil[3]{Department of Applied Physics, California Institute of Technology, Pasadena, California 91125, United States}
% \affil[*]{Corresponding author. Email: jang.minseok@kaist.ac.kr, chan.y.park@kc-ml2.com}
% \affil[$\dag$]{These authors contributed equally.}

% % Uncomment to override  the `A preprint' in the header
% % \renewcommand{\headeright}{arXiv}
% % \renewcommand{\undertitle}{Technical Report}
% % \renewcommand{\shorttitle}{\textit{arXiv} Template}

% %%% Add PDF metadata to help others organize their library
% %%% Once the PDF is generated, you can check the metadata with
% %%% $ pdfinfo template.pdf
% \hypersetup{
% pdftitle={Meent manuscript},
% % pdfsubject={q-bio.NC, q-bio.QM},
% pdfauthor={Yongha Kim},
% pdfkeywords={meent, RCWA, AD, Rigorous coupled-wave analysis, Automatic Differentiation, Inverse design},
% }

% \begin{document}
% \maketitle
% \begin{abstract}
% \input{chapters/abstract}
% \end{abstract}

% \keywords{Rigorous coupled wave analysis \and Fourier modal method \and Automatic differentiation \and Inverse design \and Vector modeling \and }
% % \clearpage

% % \tableofcontents

% % \clearpage
% \section{Introduction}
% \input{chapters/introduction}
% % \clearpage

% \section{Theory}
% \label{sec:theory}
% \input{chapters/theory/rcwa}

% \subsection{Structure design}
% \input{chapters/theory/modelling}
% % \clearpage

% \subsection{Fourier analysis of geometry}
% \input{chapters/theory/Fourier_transform}

% \subsection{Eigenmodes identification}
% \input{chapters/theory/eigenmode}

% \subsection{Connecting layers}
% \input{chapters/theory/TMM}

% \subsection{Enhanced Transmittance Matrix Method}
% \input{chapters/theory/ETM}

% \subsection{Topological derivative vs Shape derivative}
% \label{sec:Derivatives}
% \input{chapters/theory/shapeDerivative}

% \section{Simulation program sequence}
% \label{sec:Sequence}
% \input{chapters/sequence/sequence}
% % \clearpage

% \section{Benchmarks}
% \label{sec:Benchmark}
% \input{chapters/benchmark}


% \section{Applications}
% \label{sec:Applications}
% \input{chapters/applications/intro}

% % \subsection{Inverse design of thin film}
% % \input{chapters/application_thinFilm}
% % \clearpage

% % \subsection{Inverse design of 1D diffraction grating - topology}
% % \label{sec:1d_grating}
% % \input{chapters/applications/1D}

% \subsection{Inverse design of 1D grating - shape}
% \label{sec:1d_grating_vector}
% \input{chapters/applications/1D_shape}

% \subsection{Inverse design of 2D diffraction grating - topology}
% \label{sec:2d_grating}
% \input{chapters/applications/2D_deflector}

% % \subsection{Inverse design of 1D grating color router - topology}
% % \label{sec:1d_color_router}
% % \input{chapters/applications/color_router}

% \section{Concluding remarks}
% \label{sec:Conclusion}
% \input{chapters/conclusion}

% \printbibliography[heading=bibintoc]

% \end{document}

==> sections/manual/manual.tex <==
% \documentclass{format/ol-softwaremanual}
% \usepackage{format/meent}

% %%%%%%%%%%%%%%%%%%%%%%

% \usepackage[backend=biber, sorting=none, style=numeric-comp]{biblatex}
% % % \usepackage[backend=biber]{biblatex}
% \bibliography{references.bib}
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage[bb=boondox]{mathalfa}
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{stmaryrd}
% \usepackage{graphicx}
% % \usepackage{natbib}
% \usepackage{doi}
% \usepackage{amsmath}
% % \usepackage{romannum}
% % \usepackage{fontspec}
% \usepackage{color}
% \usepackage{multirow}

% % \usepackage{kotex}
% \pagenumbering{arabic}
% % \usepackage[affil-it]{authblk}
% \usepackage{blindtext}

% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{dirtytalk}
% \usepackage{csquotes}
% % \usepackage{cite}
% % \usepackage{setspace} \doublespacing
% \usepackage{esvect}
% % \usepackage{humanist}
% % \usepackage[T1]{fontenc}
% \usepackage{nicematrix}
% \usepackage{wrapfig}

% \setcounter{MaxMatrixCols}{12}

% \captionsetup{
%   justification=raggedright,
%   labelfont={color=black,bf},
%   font=small}
% \captionsetup[subfigure]{margin=10pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Frontmatter data; appears on title page
% % \title{Technical Document \\Template}
% \title{Meent: Electromagnetic simulation software}
% % \renewcommand\subtitle{dd}
% \subtitle{Manual}
% \version{0.9.9.1}

% \softwarelogo{\includegraphics[width=8cm]{chapters/cover/figures/meent_logo.png}}

% \teamlogo{\includegraphics[width=\textwidth]{chapters/generality/figures/aboutus.png}}

% \author[1]{Yongha Kim}
% \author[2, 3]{Sanmun Kim}
% \author[2]{Kevin Octavian}
% \author[2]{Doyoung Heo}
% \author[1]{Anthony W. Jung}
% \author[1, 2]{Chaejin Park}
% \author[2]{Jeongmin Shin}
% \author[2]{Chanhyung Park}
% \author[2]{Juho Park}
% \author[2]{Sangjun Han}
% \author[1]{Jinmyoung Lee}
% \author[1]{Seolho Kim}
% \author[2]{Min Seok Jang}
% \author[1]{Chan Y. Park}

% \affil[1]{KC Machine Learning Lab, Republic of Korea}
% \affil[2]{KAIST, Republic of Korea}
% \affil[3]{Caltech, United States}


% \input{sections/manual/cover/cover}

\begin{document}


\maketitle

\tableofcontents
\listoflistings
\newpage

\section{Briefing}
\input{sections/manual/briefing/briefing}

\section{Theory}
\label{sec:theory}
\input{sections/manual/theory/theory}
\clearpage


\section{Simulation program sequence}
\label{sec:Sequence}
\input{sections/manual/sequence/sequence}
\clearpage

\section{Benchmarks}
\label{sec:Benchmark}
\input{sections/manual/benchmarks/benchmark}
\clearpage

\section{Applications}
\label{sec:Applications}
\input{sections/manual/applications/applications}
\clearpage
% \section{Concluding remarks}
% \label{sec:Conclusion}
% \input{chapters/conclusion}

\printbibliography[heading=bibintoc]

\end{document}


==> sections/manual/theory/bin/CFT.tex <==
CFS utilizes the entire function to obtain its representation in the Fourier domain while DFS uses finite number of points(sampling points) which is limited information. 
% In RCWA, the device can be sliced into multi-layers so that each layer has its own permittivity distribution that is invariant in Z-direction(wave propagating direction). In other words, the permittivity can be considered as a piecewise constant function that varies on X and Y direction but has fixed value in Z direction.

The Fourier coefficients of CFS can be expressed as follows:

% \begin{align}
% f(x) = \sum_{n=-N}^{N} c_n \cdot \exp{\left(j \cdot 2\pi n \cdot \frac{x}{L}\right)} dx,
% \end{align}

% \begin{align} \label{equ:fourier_coeff_not-normalized}
% c_n = \frac{1}{L}\int_{x_0}^{x_0+L}f(x) \cdot \exp{\left(-j \cdot 2\pi n \cdot \frac{x}{L}\right)} dx,
% \end{align}

\begin{align} \label{equ:fourier_coeff_CFS}
c_{m, n} = \frac{1}{L_xL_y}\int_{x_0}^{x_0+L_x}\int_{y_0}^{y_0+L_y}f(x,y) \cdot \exp{\left[-j \cdot 2\pi \left(\frac{m}{L_x}x + \frac{n}{L_y} y \right)\right]} dydx,
\end{align}

where $m, n$ represents the coefficient index and $L_x, L_y$ is the period.

% To compute the Fourier coefficients, we consider the points of discontinuity in the function, denoted as $(x_0, x_1, x_2, ..., x_D)$ in X direction and $(y_0,  y_1,  y_2,  ...,  y_{D'})$ in Y direction, and the corresponding permittivity values in each region, denoted as $(\varepsilon_{11}, \varepsilon_{12}, ..., \varepsilon_{ii'}..., \varepsilon_{DD'})$. The function $f(x)$ can be calculated as a weighted sum of all permittivity (constant) terms:


% \begin{align}
% c_{m, n} &= \frac{1}{L_xL_y} \sum_{i=1}^{D_x} \sum_{i'=1}^{D_y} \int_{x_{i-1}}^{x_{i}} \int_{y_{i'-1}}^{y_{i'}} \varepsilon({x, y}) \cdot \exp{\left[-j \cdot 2\pi \left(\frac{m}{L_x} x + \frac{n}{L_y} y \right)\right]}dydx \\
% % &= \frac{1}{L_xL_y} \sum_{i'=1}^{D_y}\int_{y_{i'-1}}^{y_{i'}}  \sum_{i=1}^{D_x} \int_{x_{i-1}}^{x_{i}} \varepsilon({x, y}) \cdot \exp{\left[-j \cdot 2\pi \left(\frac{m}{L_x} x\right)\right]}dx  \cdot \exp{\left[-j \cdot 2\pi \left(\frac{m}{L_x} x\right)\right]}dy 
% % &= \frac{1}{j \cdot 2\pi mn} \sum_{i=1}^{D_x}  \sum_{i'=1}^{D_y} \left[(\varepsilon_{i+1} - \varepsilon_{i}) \cdot \exp{\left\{-j \cdot 2\pi \left(\frac{m}{L_x}x_i + \frac{n}{L_y}y_{i'}\right)\right\}}\right],
% \end{align}

% Since epsilon is 2D rect function, we can utilize separability:
% \begin{align}
% &= \frac{1}{j \cdot 2\pi mn} \sum_{i=1}^{D_x} \left[(\varepsilon_{i+1} - \varepsilon_{i}) \cdot \exp{\left\{-j \cdot 2\pi \left(\frac{m}{L_x}x_i \right)\right\}}\right] \sum_{i'=1}^{D_y} \left[
% (\varepsilon_{i'+1} - \varepsilon_{i'}) \cdot \exp{\left\{-j \cdot 2\pi \left(\frac{n}{L_y}y_{i'}\right)\right\}}\right] ,
% \end{align}


% \begin{align}
% c_n = \frac{1}{L} \sum_{i=1}^{D} \int_{x_i}^{x_{i+1}} \varepsilon_i \cdot \exp{\left(-j \cdot 2\pi n \cdot \frac{x}{L}\right)}dx
% = \frac{1}{j \cdot 2\pi n} \sum_{i=1}^{D} \left[(\varepsilon_{i+1} - \varepsilon_{i}) \cdot \exp{\left(-j \cdot 2\pi n \frac{x_i}{L}\right)}\right],
% \end{align}
% where $D$ is the number of discontinuous points.


% Continuous Fourier series, is a Fourier transform method where the entire function is utilized to obtain its image in the Fourier domain. Since the function to be transformed(f(x,y) = permittivity) is piecewise-constant, the Fourier coefficients in complex form can be express as the following [\cite{FFT-Mathematical_Methods}]):

% \begin{align}
%     f(x) = \sum_{n=-N}^{N} c_n \cdot \exp{\bigg(j \cdot 2\pi n \cdot \frac{x}{L}}\bigg) dx,
% \end{align}

% \begin{align} \label{equ:fourier_coeff_not-normalized}
%     c_n = \frac{1}{L}\int_{x_0}^{x_0+L}f(x) \cdot \exp{\bigg(-j \cdot 2\pi n \cdot \frac{x}{L}}\bigg) dx,
% \end{align}
% where N=number of Fourier order cut, n=each mode in fourier order, L=period.

% Given the points of discontinuity $(x_0, x_1, x_2, ..., x_D)$ and permittivity value in each region $(\varepsilon_1,\varepsilon_2, ..., \varepsilon_D)$, $f(x)$ can be calculated as a weighted sum of all permittivity (which is constant) terms.

% \begin{align}
%     c_n =& \frac{1}{L} \sum_{i=1}^{D}\int_{x_i}^{x_{i+1}}\varepsilon_i\cdot \exp{\bigg(-j \cdot 2\pi n \cdot \frac{x}{L}}\bigg)dx \\
%     =& \frac{1}{j \cdot 2\pi n} \sum_{i=1}^{D} \bigg[(\epsilon_{i+1}-\epsilon_{i}) \cdot \exp{(-j \cdot 2\pi n \frac{x_i}{L})}\bigg]
% \end{align}

% where D is the number of discontinuous points.



% This can be rearranged as:
% \begin{align}
%     c_n =& \frac{1}{L}\Bigg[ \int_{x_0}^{x_1}\varepsilon_1\cdot \exp{\bigg(-j \cdot 2\pi n \cdot \frac{x}{L}\bigg)}dx + \int_{x_1}^{x_2}\varepsilon_2\cdot \exp{\bigg(-j \cdot 2\pi n \cdot \frac{x}{L}\bigg)}dx + \cdots + \int_{x_{D-1}}^{x_D}\varepsilon_D\cdot \exp{\bigg(-j \cdot 2\pi n \cdot \frac{x}{L}\bigg)}dx\Bigg] \nonumber \\
%     =& \frac{1}{L}\Bigg[\frac{L}{-j \cdot 2\pi n}\bigg\{
%     \varepsilon_1 \cdot \exp{\bigg(-j \cdot 2\pi n \cdot \frac{x}{L}\bigg)}\bigg{\rvert}_{x_0}^{x_1} 
%     + \varepsilon_2 \cdot \exp{\bigg(-j \cdot 2\pi n \cdot \frac{x}{L}\bigg)}\bigg{\rvert}_{x_2}^{x_2}
%     + \cdots
%     + \varepsilon_D \cdot \exp{\bigg(-j \cdot 2\pi n \cdot \frac{x}{L}\bigg)}\bigg{\rvert}_{x_{D-1}}^{x_D}\bigg\}\Bigg] \nonumber \\
% % \end{align}
% % \begin{align}
%     =& \frac{1}{-j \cdot 2\pi n}\bigg[
%     + \varepsilon_1 \cdot \exp{(-j \cdot 2\pi n \cdot \frac{x_1}{L})} - \varepsilon_1 \cdot \exp{(-j \cdot 2\pi n \cdot  \frac{x_0}{L})} \nonumber \\
%     & \qquad \qquad \quad + \varepsilon_2 \cdot \exp{(-j \cdot 2\pi n \cdot  \frac{x_2}{L})} - \varepsilon_2 \cdot \exp{(-j \cdot 2\pi n \cdot  \frac{x_1}{L})} \nonumber \\
%     & \qquad \qquad \quad + \varepsilon_3 \cdot \exp{(-j \cdot 2\pi n \cdot  \frac{x_3}{L})} - \varepsilon_3 \cdot \exp{(-j \cdot 2\pi n \cdot  \frac{x_2}{L})} \nonumber \\
%     & \qquad \qquad \quad + \cdots \nonumber \\
%     & \qquad \qquad \quad + \varepsilon_D \cdot \exp{(-j \cdot 2\pi n \cdot  \frac{x_D}{L})} - \varepsilon_D \cdot \exp{(-j \cdot 2\pi n  \cdot  \frac{x_{D-1}}{L})} 
%     \bigg]\nonumber \\
%     %=& \frac{1}{-j \cdot 2\pi n}\bigg[(\varepsilon_1 - \varepsilon_2) \cdot \exp(-j \cdot 2\pi nx_1) +(\varepsilon_2 - \varepsilon_3) \cdot \exp(-j \cdot 2\pi nx_2) + \cdots +(\varepsilon_{D} - %\varepsilon_{1}) \cdot \exp(-j \cdot 2\pi nx_D) \bigg] \nonumber \\
%     =& \frac{1}{j \cdot 2\pi n}\bigg[(\varepsilon_2 - \varepsilon_1) \cdot \exp(-j \cdot 2\pi n \cdot  \frac{x_1}{L}) +(\varepsilon_3 - \varepsilon_2) \cdot \exp(-j \cdot 2\pi n \cdot  \frac{x_2}{L}) + \cdots +(\varepsilon_{1} - \varepsilon_{D}) \cdot \exp(-j \cdot 2\pi n \cdot \frac{x_D}{L}) \bigg
%     %=& \frac{1}{j \cdot 2\pi n}\bigg[(\varepsilon_2 - \varepsilon_1) \cdot \exp(n\pi x_1) +(\varepsilon_3 - \varepsilon_2) \cdot \exp(n\pi x_2) + \cdots +(\varepsilon_{1} - \varepsilon_{D}) \cdot \exp(n\pi x_D) \bigg
%     ]
% \end{align}



% \begin{figure} % picture
%     \centering
%     \includegraphics[scale=0.8]{images/picewise-constant.png}
%     \caption{piecewise-constant function}
% \end{figure}

% \subsubsection{Convergence of RCWA calculation for different Fourier transform methods}
% We address the convergence of RCWA calculation for different Fourier transform methods. Here, a 1D metagrating deflector found in Seo et. al\cite{dongjin} is used. A simulation result from RETICOLO\cite{reticolo}, a widely used RCWA library written in MATLAB, is used as a reference. As MEENT supports DFT, improved DFT, and CFT, results from each Fourier transform methods are plotted. 

% \begin{figure}[h!] % picture
%     \centering
%     \includegraphics[scale=0.7]{images/deflector_480529.png}
%     \caption{The image of 1D diffraction metagrating on a silicon oxide substrate. The height of a silicon pillar is 325 nm.}
% \end{figure}

% As was mentioned previously, Reticolo (which uses CFT) is as for the reference and 3 methods from Meent (CFT, DFT and Improved DFT) were performed with Fourier order cut sweeping. To perform DFT and rest of the RCWA steps, input size of pattern should be larger or equal to $ 2* (2*fourier\_order + 1)$(This should be $ 4*fourier\_order +1$. Check!) in each dimension and this is done by `np.repeat` function. 

% \begin{figure} % picture
%     \centering
%     \includegraphics[scale=0.7]{images/convergence.png}
%     \caption{Convergence tests of different RCWA implementations. Deflection efficiencies of -1, 0, +1 order modes are evaluated for different number of truncation Fourier orders.}
%     \label{fig:convergence}
% \end{figure}

% Convergence test of different RCWA implementation is shown in Fig. \ref{fig:convergence}. Calculation results from RETICOLO, MEENT CFT, MEENT improved DFT all agree with each other while MEENT DFT shows a result which deviates from the other three. The slow convergence of DFT is expected to originate from inaccurate Fourier transform results as discussed in Fig. \ref{fig:aliasing}.

% % \begin{figure} % picture
% %     \centering
% %     \includegraphics[scale=0.7]{images/fourier_coefficients.png}
% %     \caption{Convergence test with different Fourier\_order.}
% %     \label{fig:fourier_coefficients}
% % \end{figure}


% \begin{figure} % picture
%     \centering
%     \includegraphics[scale=0.7]{images/fourier_coefficients_difference.png}
%     \caption{Convergence test with different Fourier\_order.}
%     \label{fig:fourier_coefficients_difference}
% \end{figure}


% Fourier coefficients are plotted in fig. \ref{fig:fourier_coefficients}. Can't see anything so we add fig. \ref{fig:fourier_coefficients_difference} another plot of difference. The difference between CFT and DFT are spread over the area while CFT and DFT-improved is centered near 0.

% This doesn't necessarily mean that DFT is always bad with smaller Fourier order cut. Sometimes at small Fourier order(before converged) DFT can show closer result to converged result compared to CFT as in the example below. I consider this with the concept coherence. If Discretization frequency is well matched

==> sections/manual/theory/bin/DFT.tex <==

% Discrete Fourier transform (DFT) is the widely used choice in mapping the design to the reciprocal space. In DFT, the function, $f(x)$, to be transformed, is sampled at finite number of points. The coefficients of DFT is given by:
% \begin{equation}
%     c_n = \frac{1}{P}\sum_{i=0}^{P-1}f_i \exp{\frac{-j \cdot 2 n x_i}{P}},
% \end{equation}

% where P is the number of samples(array size), $f_i$ is the $i$th element of permittivity array, $n$ is specific Fourier order. \cite{Kreyszig}

% Performance of DFT is determined by the number of sampling points $P$, and number of Fourier orders $N$. MEENT provides an option to adjust scaling factor for geometry, which increases the resolution of the permittivity matrix by repeating its element. This option improves the geometry in the reciprocal domain and leads to a better RCWA results. Also, improving the resolution of the device can avoid geometry being aliased as described in  Nyquist–Shannon sampling theorem.

% We observe the effect of repeating the element and enhancing the device geometry by fourier transforming the geometry and inverse fourier transforming the back to the real space. $c_{10}$ and $c_{40}$ in Fig. \ref{fig:aliasing} are 10th and 40th elements in coefficients array. Now lets see how $\exp{j\cdot \frac{i}{P}}$ changes by increasing P from 200 to 2000.

% \begin{figure}[h!] % picture
%     \centering
%     \includegraphics[scale=0.6]{images/dft-10-40order.png}
%     \caption{Geometry of 2-dimensional grating layer and incident ray}
%     \label{fig:aliasing}
% \end{figure}

% \begin{figure}[h!] % picture
%     \centering
%     \includegraphics[scale=0.6]{images/dft-10-40order.png}
%     \caption{Geometry of 2-dimensional grating layer and incident ray}
%     \label{fig:aliasing}
% \end{figure}


% The Discrete Fourier Series (DFS) is a widely used method to map the device geometry to reciprocal space. 
In DFS, the function $f(x)$ to be transformed is sampled at a finite number of points. The coefficients of the DFS, denoted as $c_{m,n}$, are given by the equation:

% \begin{equation}
% c_n = \frac{1}{P}\sum_{i=0}^{P-1}f_i \exp{\left(\frac{-j \cdot 2\pi n x_i}{P}\right)},
% \end{equation}

\begin{equation}
c_{m,n} = \frac{1}{P_xP_y}\sum_{i=0}^{P_x-1}\sum_{i'=0}^{P_y-1}f_{i,i'} \exp{\left[-j \cdot 2\pi \left(\frac{m}{P_x} i + \frac{n}{P_y} i' \right)\right]},
\end{equation}

where $P_x, P_y$ are the sampling frequency (the size of the array), $f_{i,i'}$ is the element index of the permittivity array, $m, n$ are the specific diffraction order, and $j$ represents the imaginary unit.

The performance of DFS is influenced by two main factors: the number of sampling points $P_x, P_y$ and the number of Fourier Truncation Order(FTO) $M, N$. In Meent, a scaling factor for geometry is provided, which increases the resolution of the permittivity matrix by repeating its elements. This option improves the representation of the geometry in the reciprocal domain and results in better RCWA simulations.

% by preventing aliasing of the geometry, as described in the Nyquist–Shannon sampling theorem.

% Fig. \ref{fig:aliasing} is an example of aliasing in Fourier analysis. Cosine function was given with two different spatial frequencies: 2000 and 200.

% cosine function in a frequency of B/2pi

% To observe the effect of repeating the elements and enhancing the device geometry, the process involves Fourier transforming the geometry and then inverse Fourier transforming it back to the real space. In Fig. \ref{fig:aliasing}, the coefficients $c_{10}$ and $c_{40}$ are the 10th and 40th elements in the coefficients array. The impact of increasing the number of sampling points $P$ from 200 to 2000 is then observed on the behavior of $\exp(j\cdot \frac{i}{P})$.

% The results of this investigation will provide insights into the benefits of using DFT and the importance of geometry scaling in improving the performance and accuracy of RCWA simulations in MEENT.



==> sections/manual/theory/bin/rcwa_1.tex <==

%Electromagnetic field inside a periodic system can be expressed as a superposition of eigenmodes propagating inside system. RCWA solves the Maxwell's equation by identifying the eigenmodes of each layer and analysing the energy transfer between the eigenmodes of neighbouring layers. In the methods section we explain how RCWA is implemented in MEENT by dissecting the calculation process into four steps: (1) Design modelling, (2) Fourier transform of geometry, (3) Eigenmode identification, (4) Transfer matrix method. 


%이 줄에 있는 내용들은 method 맨 첫 문단에 들어가야 할 것 같아요. 기본적으로 RCWA는 z 방향으로 변하지 않는 레이어에 대해 아이겐모드를 구한 후 입사층과 투과층을 포함해 연결해 나가는 과정입니다. 각 레이어에 존재하는 전자기장과 유전율을 푸리에 스페이스로 보낸 뒤 컨벌루션을 통해 맥스웰 방정식을 풀어 각 방향의 필드에 대한 일반해를 구하게 됩니다. 이 일반 해는 아이겐분해를 통해 아이겐모드로 분해가 되며 여기에서의 fourier order에 따라 convergence가 결정됩니다. 이렇게 구해진 아이겐 모드는 진행방향 성분을 지수텀으로 갖게 되며 이를 이용해 경계면에서의 값을 구하고 레이어와 레이어를 연결합니다. 이 연결 과정에도 여러 방식이 존재하는데 대표적으로 TMM 방식과 SMM 방식이 있습니다. 두 방식 모두 같은 결과를 추구하지만 구현 방식에 차이가 있기 때문에 numerical한 차이를 갖게 됩니다. [파이라마에서 다루나?] 입사층과 투과층까지 이어주면 최종적으로 니어필드에 대한 투과효율과 반사효율을 얻게 됩니다. 이후 각 레이어에서의 필드는 경계조건을 풀면서 구한 변수들을 사용해 복원할 수 있습니다.


Inside a periodic system, the electromagnetic field can be represented as a superposition of eigenmodes that propagate within the system. To solve Maxwell's equations in such systems, RCWA follows a process of identifying the eigenmodes within each layer and analyzing the energy transfer between the eigenmodes of adjacent layers.

The methods section of the paper provides a comprehensive explanation of how RCWA is implemented in Meent. This implementation is broken down into four key steps:

\begin{enumerate}
  \item Design modeling: In this step, the device geometry is defined and modeled within the MEENT framework.
  \item Fourier transform of geometry: The device geometry is transformed into the Fourier domain, allowing the decomposition of the structure into its corresponding spatial frequency components.
  \item Eigenmode identification: MEENT then identifies the eigenmodes present within each layer of the periodic structure. These eigenmodes represent the possible electromagnetic field solutions that can exist within the system.
  \item Transfer Matrix Method: Finally, the energy transfer between the eigenmodes of neighboring layers is analyzed using the transfer matrix method. This step enables the determination of the overall electromagnetic response of the entire periodic system.

\end{enumerate}


==> sections/meent_framework/bin/meent_framework_backup.tex <==
In-depth details are available in our manual on arXiv \cyp{cite}. Here, we'll provide a concise overview of key features.


\subsection{Modeling: Raster and Vector}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{sections/meent_framework/images/modeling-2x3.png}
    \caption{Performance test: calculation time by FTO sweep. The result is normalized by NumPy case from the same options to compare the behavior of other backends. In these plots, black dashed line is $y=1$ and the results of NumPy cases lie on this line since they are normalized by themselves.}
    \label{fig:modeling-2x3}
\end{figure}

Meent offers support for two modeling methods: Raster and Vector. Analogous to the image file system, Raster represents data as an array, while Vector utilizes a set of objects, with each object comprising vertices and edges. In mathematical terms, Raster operates within discrete space, whereas Vector operates within continuous space, as shown in Fig. \ref{fig:modeling_type}. 
Due to their distinct formats, each method employs different algorithms for space transformation, resulting in different type of geometry derivatives as in Fig. \ref{fig:topology derivate} and \ref{fig:shape derivate}.

Geometry derivative, based on backpropagation through AD,
is a key feature in elevating Meent from a mere simulator to a comprehensive solution provider.
The differentiability of Meent enables automatic differentiation tracing of computational chains from input parameters to objective, facilitating the effective update of input parameters leveraging gradients derived from backpropagation.

These two modeling methods yield distinct strengths and are suited to different applications - Raster for metasurface design and Vector for OCD.

Metasurface design is the realm of device optimization that typically using Raster type devices consisting of two materials. 
The process involves iteratively flipping cells to find the optimal structure, where gradients may help effectively choose which cell to flip.
The conventional method for gradient computation in Raster type is the Adjoint method, employing adjoint sources with Lorentz reciprocity. In the context of RCWA, this method requires two RCWA simulations with field reconstruction. However, with backpropagation in Meent, reducing simulation time to one RCWA simulation and one backpropagation step.
Additionally, backpropagation serves as the only solution for finding gradients in certain applications, such as meta color router, where defining adjoint sources is not feasible.

OCD involves estimating the dimensions of specific design parameters, such as width or height of a cuboid, in devices under fabrication, aligning naturally with Vector modeling and shape derivative. Unlike Raster modeling, where dimensions are confined to discrete space, Vector modeling operates in continuous space, offering higher modeling resolution and mitigating the limitations imposed by discretization.
To the best of our knowledge, Meent stands out as the only open-source Python code supporting Vector modeling with shape derivative.

% % \begin{minipage}{\textwidth}
%     % \setlength{\columnsep}{0pt}%
%     \setlength{\intextsep}{0pt}%
%     \begin{wrapfigure}{r}{0.5\textwidth}% picture
%         % \captionsetup[subfigure]{margin=15pt}
%         \centering
%         \hfill
%         \begin{subfigure}{0.45\linewidth}   
%             \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/raster.png}
%             \caption{Raster}
%             \label{fig:raster}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.45\linewidth}   
%             \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/vector.png}
%             \caption{Vector}
%             \label{fig:vector}
%         \end{subfigure}
%         \hfill
%         \caption{\textbf{Raster versus Vector.} The blue double line denotes the codomain, while the red line represents the range. Note: In the Raster model, the resolution limits the extent of model updates achievable using automatic differentiation (AD).
%         }
%         \label{fig:modeling_type}
%     \end{wrapfigure}
    
%     Meent offers support for two modeling methods: Raster and Vector. Analogous to the image file system, Raster represents data as an array, while Vector utilizes a set of objects, with each object comprising vertices and edges. In mathematical terms, Raster operates within discrete space, whereas Vector operates within continuous space, as shown in Fig. \ref{fig:modeling_type}. Due to their distinct formats, each method employs different algorithms for space transformation, resulting in unique strengths and suitable applications.

%     From an application standpoint, Raster modeling is commonly employed in metasurface research. This method typically involves flipping each pixel to generate a freeform pattern composed of two materials. Conversely, Vector modeling finds extensive use in OCD, particularly in industrial settings. Its main objective is to determine the dimensions of design parameters, such as pitch and thickness of each layer.

% \subsection{Model update using gradient}


% % \begin{minipage}{\textwidth}
%     % \setlength{\columnsep}{0pt}%
%     \setlength{\intextsep}{0pt}%
%     \begin{wrapfigure}{r}{0.5\textwidth}% picture
%         % \captionsetup[subfigure]{margin=15pt}
%         \centering
%         \hfill
%         \begin{subfigure}{0.45\linewidth}   
%             \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/gradient-raster.png}
%             \caption{Raster}
%             \label{fig:raster}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.45\linewidth}   
%             \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/gradient-vector.png}
%             \caption{Vector}
%             \label{fig:vector}
%         \end{subfigure}
%         \hfill
%         \caption{\textbf{Raster versus Vector.} The blue double line denotes the codomain, while the red line represents the range. Note: In the Raster model, the resolution limits the extent of model updates achievable using automatic differentiation (AD).
%         }
%         \label{fig:modeling_type}
%     \end{wrapfigure}
    
    
%     One of the advantage of Meent is back-propagation (backprop). It is wide spread due to deep learning, which utilizes automatic differentiation to update the input parameters. This makes meent not just a simulator but an solution provider with optimization.
    
%     Then where is this gradient used? lets see some examples in real world.
    
%     Metasurface design is the realm of device optimization. Raster typed, two materials consisting device structure is an input, and to find the way to optimize it by flipping the cell, gradient with respect to the efficiency is used to select the cell to flip. Adjoint method is a conventional method to find gradient for each cell which uses adjoint sources using lorents reciporicity. In RCWA, It entails two RCWA simulations plus field reconstruction. With meent, backprop is available which reduces the simulation time to one RCWA plus one backprop. Other than the merit of throughput, the critical one is that meent can be used for cases that adjoint method cannot be used as color filter design. 
    
%     Above is the benefit of meent in raster type. lets see vector type which is,
%     to the best of our knowledge, meent is the only open source python code supporting automatic differentiation for Vector modeling. 
%     OCD is a domain that estimates the dimensions of specific design parameters in device under fabrication. this naturally connects to vector modeling which deals with dimensions as input. Regarding dimension, raster have to lies on discrete space while vector does in continuous space. the modeling resolution in raster is severly damaged by discretization. Vector comes to rescue.


% \clearpage
% \input{sections/meent_framework/modeling}
% \clearpage
% \end{minipage}

% \subsection{Accessibility}
% Having support for Numpy, JAX and Torch as a backend, users dont have to learn their non main framework to use meent for their experiment.


% Expandability

% Meent can be combined with Ray for distributed computing as well as RL. Can utilize GPU and TPU on ML framework.  For example 

% modularity

% Codes are organized in a modularized manner so user can easily replace any part of the process to evaluate their algorithms.

==> sections/meent_framework/bin/meent_framework_old.tex <==
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{sections/meent_framework/images/meent-overview.png}
%     \caption{Performance test: calculation time by FTO sweep. The result is normalized by NumPy case from the same options to compare the behavior of other backends. In these plots, black dashed line is $y=1$ and the results of NumPy cases lie on this line since they are normalized by themselves.}
%     \label{fig:benchmark/backend}
% \end{figure}

Regarding the details, refer our manual from arXiv. Here, only some important features will be briefly introduced.
\subsection{Modeling: topology vs shape}

% \begin{minipage}{\textwidth}
    % \setlength{\columnsep}{0pt}%
    \setlength{\intextsep}{0pt}%
    \begin{wrapfigure}{r}{0.5\textwidth}% picture
        % \captionsetup[subfigure]{margin=15pt}
        \centering
        \hfill
        \begin{subfigure}{0.45\linewidth}   
            \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/raster.png}
            \caption{Raster}
            \label{fig:raster}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.45\linewidth}   
            \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/vector.png}
            \caption{Vector}
            \label{fig:vector}
        \end{subfigure}
        \hfill
        \caption{Raster and Vector. Blue doubled line is codomain, Red is range.
        }
        \label{fig:modeling_type}
    \end{wrapfigure}
    
    Meent supports two modeling methods: Raster and Vector. As in the image file system, Raster is an array and Vector is a set of objects where each object is composed of vertices and edges. In mathematical saying, Raster is on discrete space and Vector is continuous space. Since these have different format, they have different algorithms for space transformation that leads to their own strength and proper applications. 
    
    % Algorithm-wise, Raster uses Discrete Fourier Series for transformation. This is intuitive since the input is array, as is the most data in digital computers.
    % On the other hand, Vector uses piecewise-constant Fourier series (we call this Continuous Fourier Series, CFS) thanks to the special constraint in RCWA.
    
    Application point of view, Raster is widely used for metasurface research. It is usually flip each pixel to generate freeform pattern composed of two materials. For Vector, Optical Critical Dimension is lucrative, strongly used one in industry. Its primary goal is to find the dimension of design parameters such as pitch and thickness of each layer. Consider this: if we want to find the dimensions of parameters using AD in Rater model, the amount of model update is limited by the resolution.
% \end{minipage}

% Meent supports two modeling methods: Raster and Vector. As in the image file system, Raster is an array and Vector is a set of objects where each object is composed of vertices and edges. In mathematical saying, Raster is on discrete space and Vector is continuous space. Since these have different format, they have different algorithms for space transformation that leads to their own strength and proper applications. 

% Algorithm-wise, Raster uses Discrete Fourier Series for transformation. This is intuitive since the input is array, as is the most data in digital computers.
% On the other hand, Vector uses piecewise-constant Fourier series (we call this Continuous Fourier Series, CFS) thanks to the special constraint in RCWA.

% Application point of view, Raster is widely used for metasurface research. It is usually flip each pixel to generate freeform pattern composed of two materials. For Vector, Optical Critical Dimension is lucrative, strongly used one in industry. Its primary goal is to find the dimension of design parameters such as pitch and thickness of each layer. Consider this: if we want to find the dimensions of parameters using AD in Rater model, the amount of model update is limited by the resolution.


% AD enables the calculation of the gradient of the Figure of Merit (FoM) with respect to the design parameters of the device. 

% AD in Meent can handle both modeling type - Raster and Vector - with two different forms: topological derivative and shape derivative. 

% Meent supports both topological and shape derivatives through AD.
% AD has two different forms depending on the modeling type of the geometry: topological derivative and shape derivative. 


% If the Raster modeling is utilized to obtain the geometry of the device, the gradients with respect to the refractive index of every pixel can be obtained through AD. This type of AD is known as the topological derivative, as the device design is updated pixel-wise and the topology is not conserved (Fig. \ref{fig:schematic for shape and topology derivatives}a).
% On the contrary, a shape derivative is effective for Vector modeling; the FoM derivative with respect to input dimensions is obtained as depicted in Fig. \ref{fig:schematic for shape and topology derivatives}b. The shape derivative is expected to be useful for cases where the device topology is known, but dimensions of specific structures, such as the radius of a cylinder in a layer or width and length of a cuboid, are to be found by optimization.

% Meent, to the best of our knowledge, is the only open-source RCWA library that supports direct shape derivatives with backpropagation functions. Previous publications, such as TORCWA \cite{torcwa}, support shape derivatives by assigning non-binary values to the grid cells on the boundary. This circumvents the problem of the minimum feature size being bounded by grid size and, therefore, enables the approximate calculation of shape derivatives.

% Topological derivative and shape derivative in Python are implemented differently. The pixel derivative is directly applicable from the backpropagation function provided in PyTorch and JAX libraries, as the discrete Fourier series of geometries was done using the natively supported FFT functions. However, since the geometry obtained using Vector modeling method utilizes the analytically calculated continuous Fourier series, FFT and related AD functions from PyTorch or JAX cannot be used.

% The existence of analytical differentiation results mapping the Fourier components to real components limits the applicability of the shape derivative. 

\subsection{Electromagnetic simulation}
In one sentence, RCWA is a process solving PDEs, Maxwell's equations, in Fourier space to find the optical characteristics, such as diffraction efficiency or field distribution, of the interaction between light and environment. 
We will consider two of four Maxwell's equations for RCWA simulation,
Mathematically, it is a way to find solutions for below PDEs - Eqs. \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4},
\begin{align}
    \label{eqn:maxwell 3}
    \nabla \times \mathbf E &= -j\omega\mu_0\mathbf H, \\
    \label{eqn:maxwell 4}
    \nabla \times \mathbf H &= j\omega\varepsilon_0\varepsilon_r\mathbf E,
\end{align}
% to find the electric and magnetic field inside the grating layer - $\mathbf E_g$ and $\mathbf H_g$.

% Since RCWA is a technique that solves Partial Differential Equations (PDEs), Maxwell's equations, in the Fourier space, curl operator in real space becomes multiplication and multiplication in real space becomes the convolution operator. For this convolution operation, the full set of the modes of the fields and the geometry are required so we introduce a vector notation in the subscript to denote it's a vector with all the harmonics in use, i.e.,
that describe the behavior of E and H field in real space. $\omega$ is the angular frequency, $\mu_0$ is the vacuum permeability, $\varepsilon_0$ is the vacuum permittivity, $\varepsilon_r$ is the relative permittivity.
 
These are in real space, and to change the space from real to Fourier, curl and multiplication in real space is changed into multiplication and convolution, each.

This process involves couple of mathematical techniques that scientific ML researchers are familiar with and interested in. For this reason,
Meent can be a great tool to develop and verify their ideas since RCWA encompasses interesting mathematical techniques such as Fourier analysis, convolution, eigendecomposition, etc., that are favorable topics in scientific ML community. One may try to replace or enhance these steps with machine learning. We will briefly mention them here.

\paragraph{Fourier analysis}
This is used many times in computer vision because it can capture the important features only with much smaller data size and handle the noises. In SciML community, it's getting hot after zongyi showed her work on Neural operators with FT. This applies RCWA as well. The simulation can be done is a more compressive way than other EM simulation algorithms such as FDTD and FEM. 

Simply, Fourier analysis can be expressed 
% In RCWA, the device geometry needs to be mapped to the Fourier space using Fourier analysis. To achieve this, the device is sliced into multi-layers so that each layer has Z-invariant (layer stacking direction) permittivity distribution. In other words, the permittivity can be considered as a piecewise-constant function that varies in X and Y but not Z direction in each layer. Then the geometry in real space can be expressed as a weighted sum of truncated Fourier basis 
% \begin{align}\label{eqn:fourier_series}
% \varepsilon(x, y) = \sum_{m=-\infty}^{\infty} \sum_{n=-\infty}^{\infty} c_{n, m} \cdot \exp{\left[j \cdot 2\pi \left(\frac{x}{\Lambda_x}m + \frac{y}{\Lambda_y}n\right)\right]},
% \end{align}
\begin{align}\label{eqn:fourier_series_truncation}
    \varepsilon(x, y) \simeq \sum_{m=-M}^{M} \sum_{n=-N}^{N} c_{n,m} \cdot \exp{\left[j \cdot 2\pi \left(\frac{x}{\Lambda_x}m + \frac{y}{\Lambda_y}n\right)\right]},
\end{align}
where $\Lambda_x, \Lambda_y$ are the period and $c_{n,m}$ is the Fourier coefficients, and $M, N$ are the Fourier Truncation Order (FTO) in the X and Y direction, and these can be considered as hyperparameters that affects the simulation accuracy.
Here, $c_{n,m}$ is the transformed permittivity distribution that exist in the Fourier space.
As said, this can be achieved by either DFS or CFS.


% \textbf{Convolution}
%  This part transforms the structure from the real space to the Fourier space and returns a convolution matrix (also called Toeplitz matrix) of the Fourier coefficients to apply convolution operation with the E and H fields. Fig. \ref{fig:Fourier_coeff_and_convolution} shows the Fourier coefficients matrix and convolution matrix made from the coefficient matrix.
 
% \textbf{Eigendecomposition}
% % EM fields in grating layer can be found by eigendecomposition. 
% Playing around with \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} results in second order matrix equation in the form of
% \begin{align}
%     \label{eqn:curlyS-omega_LR}
%     \boldsymbol{Q}
%     \boldsymbol{\Lambda}^2
%     =
%     \boldsymbol{\Omega}^2
%     \boldsymbol{Q}
% \end{align}


% \begin{align}
%     \label{eqn:curlyS-omega_LR}
%     \Lambda^2
%     \begin{bmatrix}
%     \boldsymbol{E_x} \\
%     \boldsymbol{E_y}
%     \end{bmatrix}
%     =
%     \boldsymbol{\Omega}^2
%     \begin{bmatrix}
%     \boldsymbol{E_x} \\
%     \boldsymbol{E_y}
%     \end{bmatrix}
% \end{align}
% Here Ex and Ey can be found by eigendecomposition. This is the most time-consuming part in RCWA and a hurdle to adopt GPU as a main device for RCWA. To save time, there have been many researched trying to replace this with NN. Some showed great performance but they were on hermitian matrices while ours is non-hermitian.

\textbf{Eigendecomposition}
Playing around with \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} results in second order matrix equation
\begin{align}
    \label{eqn:curlyS-omega_LR}
    (-j\tilde{k}_{g,z})^2
    \begin{bmatrix}
    \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
    \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
    \end{bmatrix}
    =
    \boldsymbol{{\Omega}}_{g,LR}^2
    \begin{bmatrix}
    \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
    \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
    \end{bmatrix},
\end{align}
where
\begin{align}
    \label{eqn:omega_LR}
    \boldsymbol{{\Omega}}_{g,LR}^2 =
    \begin{bmatrix}
    {\tilde{\mathbf K}_y}^2 + (\tilde{\mathbf{K}}_x \llbracket\varepsilon_{r,g}\rrbracket^{-1} \tilde{\mathbf{K}}_x - \mathbf{I}) \llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1} 
    & \tilde{\mathbf K}_x(\llbracket\varepsilon_{r,g}\rrbracket^{-1}\tilde{\mathbf K}_y\llbracket\varepsilon_{r,g}\rrbracket - \tilde{\mathbf K}_y) \\
    \tilde{\mathbf K}_y(\llbracket\varepsilon_{r,g}\rrbracket^{-1}\tilde{\mathbf K}_x\llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1} - \tilde{\mathbf K}_x) 
    & {\tilde{\mathbf K}_x}^2 + (\tilde{\mathbf{K}}_y \llbracket\varepsilon_{r,g}\rrbracket^{-1} \tilde{\mathbf K}_y - \mathbf{I})\llbracket\varepsilon_{r,g}\rrbracket
    \end{bmatrix}.
\end{align}
This omega matrix is composed of wavevector matrices and permittivity map in Fourier space. $\llbracket\ \rrbracket$ is the convolution (a.k.a Toeplitz) matrix: $\llbracket\varepsilon_{r,g}\rrbracket$ and $\llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1}$ are convolution matrices composed of Fourier coefficients of permittivity and one-over-permittivity (by the inverse rule presented in \cite{Li:96} and \cite{Li:hal-00985928}).
This is simply
% \(Q \Lambda^2 = \Omega^2 Q\)
\begin{align}
    \label{eqn:curlyS-omega_LR}
    \boldsymbol{Q}
    \boldsymbol{\Lambda}^2
    =
    \boldsymbol{\Omega}^2
    \boldsymbol{Q}
\end{align}
that can be solved with eigendecomposition.
Recently there are studies that using ML to find eigenvalues [] []. But those are limited to hermitian cases while ours is non-hermitian.
Here Ex and Ey can be found by eigendecomposition. This is the most time-consuming part in RCWA and a hurdle to adopt GPU as a main device for RCWA. To save time, there have been many researched trying to replace this with NN. Some showed great performance but they were on hermitian matrices while ours is non-hermitian.

\textbf{Boundary condition} Like PDEs in PINN have boundary conditions, RCWA is also applied. Let's say there are two layers that facing each other. E field of the first layer at the boundary should be matched to the E field of the second layer at the boundary. H field as well, and this can be written in matrix form

% This equation for a single layer grating can be simply extended to a multi-layer system as the following:
% \begin{align}
%     \label{eqn:solve-multilayer}
%     \begin{bmatrix}
%         \sin\psi\ \boldsymbol\delta_{00} \\
%         \cos\psi\ \cos\theta\ \boldsymbol\delta_{00}
%          \\
%         j\sin\psi\ \mathtt n_{\text{I}} \cos\theta\ \boldsymbol\delta_{00} \\
%         -j\cos\psi\ \mathtt n_{\text{I}}\ \boldsymbol\delta_{00} \\
%     \end{bmatrix}
%     +
%     \begin{bmatrix}
%         \mathbf I & \mathbf 0 \\
%         \mathbf 0 & -j\mathbf Z_I \\
%         -j\mathbf Y_I & \mathbf 0 \\
%         \mathbf 0 & \mathbf I
%     \end{bmatrix}
%     \begin{bmatrix}
%         \mathbf R_s \\
%         \mathbf R_p
%     \end{bmatrix}
%     % \\\quad\\
%     % \begin{align*}
%     =
%     \prod_{\ell=1}^{L}
%     \begin{bmatrix}
%     \mathbb W_\ell & \mathbb {W_\ell X_\ell} \\
%     \mathbb V_\ell & -\mathbb {V_\ell X_\ell}
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbb {W_\ell X_\ell} & \mathbb W_\ell \\
%     \mathbb {V_\ell X_\ell} & -\mathbb V_\ell
%     \end{bmatrix}^{-1}
%     \begin{bmatrix}
%     \mathbb F_{L+1} \\
%     \mathbb G_{L+1} \\
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbf T_s \\ \mathbf T_p
%     \end{bmatrix},
%     % \end{align*}
% \end{align}
% where $L$ is the number of layers.

\begin{align}
    \label{eq:bc}
    \begin{bmatrix}
        \sin\psi\ \boldsymbol\delta_{00} \\
        \cos\psi\ \cos\theta\ \boldsymbol\delta_{00}
         \\
        j\sin\psi\ \mathtt n_{\text{I}} \cos\theta\ \boldsymbol\delta_{00} \\
        -j\cos\psi\ \mathtt n_{\text{I}}\ \boldsymbol\delta_{00} \\
    \end{bmatrix}
    +
    \begin{bmatrix}
        \mathbf I & \mathbf 0 \\
        \mathbf 0 & -j\mathbf Z_I \\
        -j\mathbf Y_I & \mathbf 0 \\
        \mathbf 0 & \mathbf I
    \end{bmatrix}
    \begin{bmatrix}
        \mathbf R_s \\
        \mathbf R_p
    \end{bmatrix}
    % \\\quad\\
    % \begin{align*}
    =
    \begin{bmatrix}
    \mathbb W & \mathbb {W X} \\
    \mathbb V & -\mathbb {V X}
    \end{bmatrix}
    \begin{bmatrix}
    \mathbb {W X} & \mathbb W \\
    \mathbb {V X} & -\mathbb V
    \end{bmatrix}^{-1}
    \begin{bmatrix}
    \mathbb F \\
    \mathbb G \\
    \end{bmatrix}
    \begin{bmatrix}
    \mathbf T_s \\ \mathbf T_p
    \end{bmatrix},
    % \end{align*}
\end{align}
% and
% \begin{align}
%     \mathbb F_{L+1}
%     =
%     \begin{bmatrix}
%     \mathbf I & \mathbf 0 \\
%     \mathbf 0 & j\mathbf Z_{\text{II}}
%     \end{bmatrix}, \quad
%     \mathbb G_{L+1}
%     =
%     \begin{bmatrix}
%     j\mathbf Y_{\text{II}} & \mathbf 0 \\
%     \mathbf 0 & \mathbf I
%     \end{bmatrix}.
% \end{align}
Since we have four matrix equations for four unknown coefficients ($\mathbf R_s, \mathbf R_p, \mathbf T_s, \mathbf T_p$), they can be derived and used for calculating diffraction efficiencies (also called the reflectance and transmittance).

% \subsection{Automatic Differentiation}
% For the optimization, we will use the gradient to select the cell to flip, and this will be calculated by AD instead of adjoint method which is commonly used technique in Metasurface design. As well explained in \cite{jlab-review}, adjoint method greatly reduces the number of needed calculations from the twice of the number of design parameters to only two.
% % (e.g., a 2D pattern with the resolution of 256x256 pixels needs 256x256 + 1 RCWA simulations to find gradient per each cell but adjoint method needs only 2 simulations). 
% However, this can be further improved with AD. It takes one RCWA simulation and one backward pass (a.k.a. backpropagation) which is computationally cheaper as shown in Fig. \ref{fig:ad-all}b.


% \subsection{Backend: NumPy, JAX and PyTorch}
% Meent is served on multiple backends. Users don't have to change their codes to use Meent. 

% \textbf{NumPy\quad} This is easy to use with limited functionalities of Meent. This is recommended for small size of problem that does not need AD and GPU device.

% \textbf{JAX\quad} JAX is newly deveploed ML framework from google. Its famous feature is jit compilation and pmap. These are fully supported in Meent. Especially pmap shows huge impact in spectrum calcultion which repeates the same calculation by sweeping wavelength. Recommended for heavy and experienced users. 

% \textbf{PyTorch\quad} Mostly beloved ML framework. Easy to use. Low hurdle for coding - not like JAX which has grammatical constraints due to jit compilation. 

% % NumPy, JAX and PyTorch as a backend are benchmarked. NumPy is installed via PyPI which is compiled with OpenBLAS. There are many types of BLAS libraries and the most representative ones are OpenBLAS and MKL (Math Kernel Library).
% % As of now, PyPI provides NumPy with OpenBLAS while conda does one with MKL. This makes small discrepancy in terms of speed and precision hence pay attention when doing consistency test between machines.

% Please refer our manual in arXiv for more information. It provides computing performance evaluation with all conditions.

\subsection{\textcolor{red}{examplary FoM: efficiency and e field}}

maybe put deflection efficiency equation and E field equation here and refer to the python method \verb|meent.get_efficiency|, \verb|meent.get_efield|

Electric field ($E$) can be found by substituting  \eqref{eqn:maxwell 4} into \eqref{eqn:maxwell 3},
\begin{equation}
    \label{eq:pde}
    \nabla\times\nabla\times E(x,y,z) = \omega^2 \mu_0 \varepsilon_0 \varepsilon_r E(x,y,z)
\end{equation}
where $\omega$ is the angular frequency, $\mu_0$ is the vacuum permeability, $\varepsilon_0$ is the vacuum permittivity, $\varepsilon_r$ is the relative permittivity and $x, y, z$ is the spatial coordinates.


% \textbf{Computing performance}
% In this section, computing options to speed up the calculation - backend, device (CPU and GPU) and architecture (64bit and 32bit) - will be benchmarked. Table \ref{tab:hardware} is the hardware specification of the test server and Table \ref{tab:performance_condition} is the index of each test condition.

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\textwidth]{images/benchmarks/performance/result_all.png}
% %     \caption{Performance test: calculation time with respect to FTO. Top row is the result from 64bit and bottom is from 32bit. The first column is the result from the test server alpha and the rest is beta and gamma in order.}
% %     \label{fig:benchmark/performance_all}
% % \end{figure}

% The graphs in Fig. \ref{fig:benchmark/performance_all} are calculation time vs FTO with all the data per machine and architecture. Before look into the details, we will briefly mention some notice in this figure. (1) JAX can't afford large FTO regardless of device. We suspect that this is related to JIT compilation which takes much time and memory for the compilation at the first run. (2) GPU with JAX and PyTorch can't accept large FTO even though GPU memory is more than needed for array upload. (3) if large amount of calculation is needed, Numpy or PyTorch on CPU is the option. (4) no golden option exists: it is recommended to find the best option for the test environment by doing benchmark tests.

% We will visit these computing options one by one. The option C9 at FTO 1600 will be excluded in further analyses: this seems an optimization issue in PyTorch or CUDA.



% \begin{table}
% \caption{Hardware specification}
% \label{tab:hardware}
% \centering
% \begin{tabular}{ l||l|l|l|l } 
% \hline
% & CPU & clock & \# threads & GPU \\
% \hline\hline
% Alpha & Intel Xeon Gold 6138 & 2.00GHz & 80 & - \\
% Beta & Intel Xeon E5-2650 v4 & 2.20GHz & 48 & GeForce RTX 2080ti \\
% Gamma & Intel Xeon Gold 6226R & 2.90GHz & 64 & GeForce RTX 3090 \\
% \hline
% \end{tabular}
% \end{table}
% \begin{center}
% \begin{table}
% \begin{center}
% \caption{Performance test condition}
% \label{tab:performance_condition}
% \begin{tabular}{ |c|c|c||c|c|c| }
% \hline
% backend & device & bit & alpha server & beta server & gamma server\\
% \hline\hline
% NumPy & CPU & 64 & (A1) & (B1) & (C1)\\ 
% NumPy & CPU & 32  & (A2) & (B2) & (C2)\\ 
% JAX & CPU & 64  & (A3) & (B3) & (C3)\\ 
% JAX & CPU & 32  & (A4) & (B4) & (C4)\\ 
% JAX & GPU & 64  & - & (B5) & (C5)\\ 
% JAX & GPU & 32  & - & (B6) & (C6)\\
% PyTorch & CPU & 64 & (A7) & (B7) & (C7)\\ 
% PyTorch & CPU & 32 & (A8) & (B8) & (C8)\\ 
% PyTorch & GPU & 64 & - & (B9) & (C9)\\ 
% PyTorch & GPU & 32 & - & (B10) & (C10)\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}
% \end{center}

% % \begin{center}
% % \begin{table}
% % \begin{center}
% % \caption{Performance test condition}
% % \label{tab:performance_condition}
% % \begin{minipage}{0.3\linewidth}
% % \begin{scriptsize}
% % \caption{Alpha server}
% % \begin{tabular}{ |c|c|c|c| }
% % \hline
% % & backend & device & bit \\
% % \hline\hline
% % (A1) & numpy & CPU & 64 \\ 
% % (A2) & numpy & CPU & 32 \\ 
% % (A3) & jax & CPU & 64 \\ 
% % (A4) & jax & CPU & 32 \\ 
% % - & jax & GPU & 64 \\ 
% % - & jax & GPU & 32 \\
% % (A7) & torch & CPU & 64 \\ 
% % (A8) & torch & CPU & 32 \\ 
% % - & torch & GPU & 64 \\ 
% % - & torch & GPU & 32 \\
% % \hline
% % \end{tabular}
% % \end{scriptsize}
% % \end{minipage}
% % \begin{minipage}{0.3\linewidth}
% % \begin{scriptsize}
% % \caption{Beta server}
% % \begin{tabular}{ |c|c|c|c| } 
% % \hline
% % & backend & device & bit \\
% % \hline\hline
% % (B1) & numpy & CPU & 64 \\ 
% % (B2) & numpy & CPU & 32 \\ 
% % (B3) & jax & CPU & 64 \\ 
% % (B4) & jax & CPU & 32 \\ 
% % (B5) & jax & GPU & 64 \\ 
% % (B6) & jax & GPU & 32 \\
% % (B7) & torch & CPU & 64 \\ 
% % (B8) & torch & CPU & 32 \\ 
% % (B9) & torch & GPU & 64 \\ 
% % (B10) & torch & GPU & 32 \\
% % \hline
% % \end{tabular}
% % \end{scriptsize}
% % \end{minipage}
% % \begin{minipage}{0.3\linewidth}
% % \begin{scriptsize}
% % \caption{Gamma server}
% % \begin{tabular}{ |c|c|c|c| } 
% % \hline
% % & backend & device & bit \\
% % \hline\hline
% % (C1) & numpy & CPU & 64 \\ 
% % (C2) & numpy & CPU & 32 \\ 
% % (C3) & jax & CPU & 64 \\ 
% % (C4) & jax & CPU & 32 \\ 
% % (C5) & jax & GPU & 64 \\ 
% % (C6) & jax & GPU & 32 \\
% % (C7) & torch & CPU & 64 \\ 
% % (C8) & torch & CPU & 32 \\ 
% % (C9) & torch & GPU & 64 \\ 
% % (C10) & torch & GPU & 32 \\
% % \hline
% % \end{tabular}
% % \end{scriptsize}
% % \end{minipage}
% % \end{center}
% % \end{table}
% % \end{center}
% In this section, computing options to speed up the calculation - backend, device (CPU and GPU) and architecture (64bit and 32bit) - will be benchmarked. Table \ref{tab:hardware} is the hardware specification of the test server and Table \ref{tab:performance_condition} is the index of each test condition.

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{sections/meent_framework/images/result_all.png}
%     \caption{Performance test: calculation time with respect to FTO. Top row is the result from 64bit and bottom is from 32bit. The first column is the result from the test server alpha and the rest is beta and gamma in order.}
%     \label{fig:benchmark/performance_all}
% \end{figure}

% The graphs in Fig. \ref{fig:benchmark/performance_all} are calculation time vs FTO with all the data per machine and architecture. Before look into the details, we will briefly mention some notice in this figure. (1) JAX can't afford large FTO regardless of device. We suspect that this is related to JIT compilation which takes much time and memory for the compilation at the first run. (2) GPU with JAX and PyTorch can't accept large FTO even though GPU memory is more than needed for array upload. (3) if large amount of calculation is needed, Numpy or PyTorch on CPU is the option. (4) no golden option exists: it is recommended to find the best option for the test environment by doing benchmark tests.

% We will visit these computing options one by one. The option C9 at FTO 1600 will be excluded in further analyses: this seems an optimization issue in PyTorch or CUDA.

% \subsubsection{Backend: NumPy, JAX and PyTorch}
% NumPy, JAX and PyTorch as a backend are benchmarked. NumPy is installed via PyPI which is compiled with OpenBLAS. There are many types of BLAS libraries and the most representative ones are OpenBLAS and MKL (Math Kernel Library).
% As of now, PyPI provides NumPy with OpenBLAS while conda does one with MKL. This makes small discrepancy in terms of speed and precision hence pay attention when doing consistency test between machines.
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{sections/meent_framework/images/backend.png}
%     \caption{Performance test: calculation time by FTO sweep. The result is normalized by NumPy case from the same options to compare the behavior of other backends. In these plots, black dashed line is $y=1$ and the results of NumPy cases lie on this line since they are normalized by themselves.}
%     \label{fig:benchmark/backend}
% \end{figure}
% Fig. \ref{fig:benchmark/backend} is the relative simulation time per server and architecture normalized by the time of NumPy case in the same conditions to make comparison easy.
% In small FTO regime, all the options were successfully operated and no champion exists. Hence it is strongly recommended to run benchmark test on your hardware and pick the most efficient one. In case of X7 (A7, B7 and C7), alpha and gamma show the same behavior - spike in 100 - while beta shows fluctuation around B1. One possible reason for this is the type of CPU. The CPUs of alpha and gamma belong to `Xeon Scalable Processors' group but Beta is `Xeon E Processors'. Currently we don't know if this actually makes difference or some other reason (such as the number of threads or BLAS implementation) does. This result may vary if MKL were used instead of OpenBLAS.
% In large FTO, only two options are available: NumPy and PyTorch on CPU in 64 bit. In case of JAX, the tests were failed: we watched memory occupation surge during the simulation which seems unrelated to matrix calculation. This might be an issue of JIT (Just In Time) compilation in JAX. Between NumPy and PyTorch, PyTorch is about twice faster than NumPy in both architectures at alpha and gamma, but beta shows different behavior. This too, we don't know the root cause but one notable difference is the family of CPU type.

% \subsubsection{Device: CPU and GPU}
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{sections/meent_framework/images/device.png}
%     \caption{Performance test result: calculation time of GPU cases are normalized by CPU cases from the same options to see the efficiency of GPU utilization. In these plots, black dashed line is $y=1$ where the capability of both are the same.}
%     \label{fig:benchmark/device}
% \end{figure}

% Fig. \ref{fig:benchmark/device} shows the relative simulation time of GPU cases normalized by CPU cases on the same backend and architecture. Note that it is \textbf{relative} time, so the smaller time does not mean it is a good option for the simulation experiments: the relative time can be small even if the absolute time of CPU and GPU are very large compared to other options.

% JAX shows good GPU utilization throughout the whole range (except one point in beta) regardless of the architecture. Considering the architecture, the data trend in beta is not clear while the gamma clearly shows that GPU utilization can be more effective in 32bit operation. PyTorch data is a bit noisier than of JAX, but has the similar behavior per server. The data in beta is hard to conclude as the JAX cases and the gamma too shows ambiguous trend but we can consider GPU option is efficient with wide range of FTOs.
% % It is also effective in PyTorch. FTO range of $200\sim800$ in beta (except one point) and $100\sim800$ in gamma show smaller simulation time with GPU utilization. Above 1600 in beta or 3200 in gamma, GPU tests failed. 

% Up to date, eigendecomposition for non-hermitian matrix which is the most expensive step ($O(M^3N^3)$) in RCWA, is not implemented on GPU in JAX and PyTorch hence the calculations are done on CPU and the results are sent back to GPU. As a result, we cannot expect great performance enhancement in using GPUs. 

% \subsubsection{Architecture: 64 and 32 bit}
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{sections/meent_framework/images/archi.png}
%     \caption{Performance test result: calculation time of 32bit cases are normalized by 64bit cases from the same options. In these plots, black dashed line is $y=1$ where the capability of both are the same.}
%     \label{fig:benchmark/archi}
% \end{figure}

% In Fig. \ref{fig:benchmark/archi}, calculation time of 32bit case is normalized by 64bit case with the same condition. With some exceptions, most points show that simulation in 32bit is faster than 64bit. Here are some important notes:
% (1) From our understanding, the eigendecomposition (Eig) in NumPy operates in 64bit regardless of the input type - even though the input is 32bit data (float32 or complex64), the matrix operations inside Eig are done in 64bit but returns the results in 32bit data type. This is different from JAX and PyTorch - they provides Eig in 32bit as well as 64bit. Hence the 32bit NumPy cases in the figure approach to 1 as FTO increases because the calculation time for Eig is the same and it is the most time-consuming step.
% (2) Keep in mind that 32bit data type can handle only 8 digits. This means that 1000 + 0.00001 becomes 1000 without any warnings or error raises. For such a reason, the accuracy of 32bit cases in the figures are not guaranteed - we only consider the calculation time.
% % (3) Eig in PyTorch shows interesting behavior. As FTO increases, Eig time in 32bit overtakes 64bit and this causes the time of B8 and C8 also increases as FTO increases. This is counter-intuitive and we don't have good explanation but cautiously presume that this might be related to the accuracy and precision in Eig or an optimization issue of PyTorch.
% (3) Eig in PyTorch shows interesting behavior: as FTO increases, calculation time in 32bit overtakes 64bit - see A8/A7, B8/B7 and C8/C7. This is counter-intuitive and we don't have good explanation but cautiously guess that this might be related to the accuracy and precision in Eig or an optimization issue of PyTorch.



==> sections/meent_framework/bin/modeling.tex <==

\subsection{Modeling: Raster and Vector}

% \setlength{\intextsep}{0pt}%
% \begin{wrapfigure}{r}{0.5\textwidth}% picture
%     % \captionsetup[subfigure]{margin=15pt}
%     \centering
%     \hfill
%     \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/modeling-2x2.png}
%     \caption{Raster}
%     \label{fig:raster}
%     \caption{\textbf{Raster versus Vector.} Two types of geometry modeling: Raster and Vector. The left of (a) and (b) show how the geometry is formed by each method and the right figures are the representative applications - metasurface design and OCD. \textbf{Geometry Derivatives.} A schematic diagram showing the difference between the (a) topological derivative and (b) shape derivative. The topological derivative results in the FoM derivative with respect to the permittivity changes of every cells in the grid and the shape derivative provides the derivative with respect to the deformations of a shape..
%     }
%     \label{fig:modeling_type}
% \end{wrapfigure}


Meent offers support for two modeling methods: Raster and Vector. Analogous to the image file system, Raster represents data as an array, while Vector utilizes a set of objects, with each object comprising vertices and edges. In mathematical terms, Raster operates within discrete space, whereas Vector operates within continuous space, as shown in Fig. \ref{fig:modeling_type}. 
Due to their distinct formats, each method employs different algorithms for space transformation, resulting in different type of geometry derivatives as in Fig. \ref{fig:topology derivate} and \ref{fig:shape derivate}.

Geometry derivative, based on backpropagation through AD,
is a key feature in elevating Meent from a mere simulator to a comprehensive solution provider.
The differentiability of Meent enables automatic differentiation tracing of computational chains from input parameters to objective, facilitating the effective update of input parameters leveraging gradients derived from backpropagation.

These two modeling methods yield distinct strengths and are suited to different applications - Raster for metasurface design and Vector for OCD.

Metasurface design is the realm of device optimization that typically using Raster type devices consisting of two materials. 
The process involves iteratively flipping cells to find the optimal structure, where gradients may help effectively choose which cell to flip.
The conventional method for gradient computation in Raster type is the Adjoint method, employing adjoint sources with Lorentz reciprocity. In the context of RCWA, this method requires two RCWA simulations with field reconstruction. However, with backpropagation in Meent, reducing simulation time to one RCWA simulation and one backpropagation step.
Additionally, backpropagation serves as the only solution for finding gradients in certain applications, such as meta color router, where defining adjoint sources is not feasible.

OCD involves estimating the dimensions of specific design parameters, such as width or height of a cuboid, in devices under fabrication, aligning naturally with Vector modeling and shape derivative. Unlike Raster modeling, where dimensions are confined to discrete space, Vector modeling operates in continuous space, offering higher modeling resolution and mitigating the limitations imposed by discretization.
To the best of our knowledge, Meent stands out as the only open-source Python code supporting Vector modeling with shape derivative.

% % \begin{minipage}{\textwidth}
%     % \setlength{\columnsep}{0pt}%
%     \setlength{\intextsep}{0pt}%
%     \begin{wrapfigure}{r}{0.5\textwidth}% picture
%         % \captionsetup[subfigure]{margin=15pt}
%         \centering
%         \hfill
%         \begin{subfigure}{0.45\linewidth}   
%             \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/raster.png}
%             \caption{Raster}
%             \label{fig:raster}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.45\linewidth}   
%             \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/vector.png}
%             \caption{Vector}
%             \label{fig:vector}
%         \end{subfigure}
%         \hfill
%         \caption{\textbf{Raster versus Vector.} Two types of geometry modeling: Raster and Vector. The left of (a) and (b) show how the geometry is formed by each method and the right figures are the representative applications - metasurface design and OCD.
%         }
%         \label{fig:modeling_type}
%     \end{wrapfigure}
    

% % \end{minipage}
% % \begin{minipage}{\textwidth}
%     % \setlength{\columnsep}{0pt}%
%     \setlength{\intextsep}{0pt}%
%     \begin{wrapfigure}{r}{0.5\textwidth}% picture
%         % \captionsetup[subfigure]{margin=15pt}
%         \centering
%         \hfill
%         \begin{subfigure}{0.45\linewidth}   
%             \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/gradient-raster.png}
%             \caption{Raster}
%             \label{fig:topology derivate}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.45\linewidth}   
%             \includegraphics[width=\linewidth, trim=1 1 1 1, clip]{sections/meent_framework/images/gradient-vector.png}
%             \caption{Vector}
%             \label{fig:shape derivate}
%         \end{subfigure}
%         \hfill
%         \caption{\textbf{Geometry Derivatives.} A schematic diagram showing the difference between the (a) topological derivative and (b) shape derivative. The topological derivative results in the FoM derivative with respect to the permittivity changes of every cells in the grid and the shape derivative provides the derivative with respect to the deformations of a shape..
%         }
%         \label{fig:modeling_type}
%     \end{wrapfigure}
    
    

==> sections/meent_framework/bin/rcwa0.tex <==

Meent uses RCWA for EM solver. It is fast algorithm to calculate the optical characteristics of environment. Due to its space change, it incorporates many skills that needs domain knowledge. Full derivation is huge so see appendix.

In one sentence, RCWA is a technique used to solve partial differential equations (PDEs), notably Maxwell's equations, in Fourier space, aiming to estimate optical properties like diffraction efficiency or field distribution, emerging from the interaction between light and its environment.

This process involves couple of mathematical techniques such as Fourier analysis, convolution, eigendecomposition, etc., that are favorable topics in scientific ML community. For this reason,
Meent can be a great tool to develop and verify their ideas. One may try to replace or enhance these steps with machine learning. 
We will introduce two most important steps that may attract ML researchers - Fourier analysis and eigendecomposition.

% It includes many steps and derivations which cannot be written here due to its size and need for domain knowledge.
% so for readers who is interested in physics, refer this and that.

% This process involves couple of mathematical techniques that scientific ML researchers are familiar with and interested in. For this reason,
% Meent can be a great tool to develop and verify their ideas since RCWA encompasses interesting mathematical techniques such as Fourier analysis, convolution, eigendecomposition, etc., that are favorable topics in scientific ML community. One may try to replace or enhance these steps with machine learning. We will briefly mention them here.

% It includes many steps and derivations which cannot be written here due to its size and need for domain knowledge.
% so we will explain bit more but as less as possible, and for readers who is interested in physics, refer this and that.

\paragraph{Fourier analysis}
%% original
% This is used many times in computer vision because it can capture the important features only with much smaller data size and handle the noises. In SciML community, it's getting hot after zongyi showed her work on Neural operators with FT. This applies RCWA as well. The simulation can be done is a more compressive way than other EM simulation algorithms such as FDTD and FEM. 

This technique is widely employed in computer vision due to its ability to compress the data - capture essential features and effective noise handling \cite{}. 
One successful example in sciML community is Fourier neural operator (FNO) \cite{} which uses Fourier analyses. \textcolor{blue}{write more}.
This concept extends to RCWA, where simulations can be conducted in a more efficient manner (under some constraints) compared to other EM simulation algorithms such as finite-difference time-domain and finite element method.

Simply, Fourier analysis can be expressed as:
\begin{align}\label{eqn:fourier_series_truncation}
    f(x, y) \simeq \sum_{m=-M}^{M} \sum_{n=-N}^{N} c_{n,m} \cdot \exp{\left[j \cdot 2\pi \left(\frac{x}{\Lambda_x}m + \frac{y}{\Lambda_y}n\right)\right]},
\end{align}
where $\Lambda_x$ and $\Lambda_y$ are the period, $c_{n,m}$ is the Fourier coefficients, and $M$ and $N$ are the Fourier truncation order (FTO) in the X and Y direction, respectively. In ML terms, $M$ and $N$ are hyperparameters that affects the simulation accuracy.

\textbf{Eigendecomposition}

% Playing around with \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} results in second order matrix equation

% Fourier analysis, then, takes input \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} and rewrite these in Fourier space. These rewritten 2 equations are combined into a single set of second order equations to find general solution.

% Eig is used to find general solution. Eqs. \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} 

% To find the field, Eqs. \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} are sent to Fourier space, and combined into a single set of second order equations as:

% Electric and magnetic field that sent to Fourier space now can be combined to a single set of second order equations

% \begin{align}
%     \label{eqn:curlyS-omega_LR}
%     (-j\tilde{k}_{g,z})^2
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
%     \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
%     \end{bmatrix}
%     =
%     \boldsymbol{{\Omega}}_{g,LR}^2
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
%     \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
%     \end{bmatrix},
% \end{align}
% where
% \begin{align}
%     \label{eqn:omega_LR}
%     \boldsymbol{{\Omega}}_{g,LR}^2 =
%     \begin{bmatrix}
%     {\tilde{\mathbf K}_y}^2 + (\tilde{\mathbf{K}}_x \llbracket\varepsilon_{r,g}\rrbracket^{-1} \tilde{\mathbf{K}}_x - \mathbf{I}) \llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1} 
%     & \tilde{\mathbf K}_x(\llbracket\varepsilon_{r,g}\rrbracket^{-1}\tilde{\mathbf K}_y\llbracket\varepsilon_{r,g}\rrbracket - \tilde{\mathbf K}_y) \\
%     \tilde{\mathbf K}_y(\llbracket\varepsilon_{r,g}\rrbracket^{-1}\tilde{\mathbf K}_x\llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1} - \tilde{\mathbf K}_x) 
%     & {\tilde{\mathbf K}_x}^2 + (\tilde{\mathbf{K}}_y \llbracket\varepsilon_{r,g}\rrbracket^{-1} \tilde{\mathbf K}_y - \mathbf{I})\llbracket\varepsilon_{r,g}\rrbracket
%     \end{bmatrix}.
% \end{align}
% This omega matrix is composed of wavevector matrices and permittivity map in Fourier space. $\llbracket\ \rrbracket$ is the convolution (a.k.a Toeplitz) matrix: $\llbracket\varepsilon_{r,g}\rrbracket$ and $\llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1}$ are convolution matrices composed of Fourier coefficients of permittivity and one-over-permittivity (by the inverse rule presented in \cite{Li:96} and \cite{Li:hal-00985928}).
This is used to find general solution 
This is simply
% \(Q \Lambda^2 = \Omega^2 Q\)
\begin{align}
    \label{eqn:eigendecomposition}
    \boldsymbol{Q}
    \boldsymbol{\Lambda}^2
    =
    \boldsymbol{\Omega}^2
    \boldsymbol{Q}
\end{align}
that can be solved with eigendecomposition.
Recently there are studies that using ML to find eigenvalues [] []. But those are limited to hermitian cases while ours is non-hermitian.
Here Ex and Ey can be found by eigendecomposition. This is the most time-consuming part in RCWA and a hurdle to adopt GPU as a main device for RCWA. To save time, there have been many researched trying to replace this with NN. Some showed great performance but they were on hermitian matrices while ours is non-hermitian.

% \textbf{Boundary condition} Like PDEs in PINN have boundary conditions, RCWA is also applied. Let's say there are two layers that facing each other. E field of the first layer at the boundary should be matched to the E field of the second layer at the boundary. H field as well, and this can be written in matrix form

% \begin{align}
%     \label{eq:bc}
%     \begin{bmatrix}
%         \sin\psi\ \boldsymbol\delta_{00} \\
%         \cos\psi\ \cos\theta\ \boldsymbol\delta_{00}
%          \\
%         j\sin\psi\ \mathtt n_{\text{I}} \cos\theta\ \boldsymbol\delta_{00} \\
%         -j\cos\psi\ \mathtt n_{\text{I}}\ \boldsymbol\delta_{00} \\
%     \end{bmatrix}
%     +
%     \begin{bmatrix}
%         \mathbf I & \mathbf 0 \\
%         \mathbf 0 & -j\mathbf Z_I \\
%         -j\mathbf Y_I & \mathbf 0 \\
%         \mathbf 0 & \mathbf I
%     \end{bmatrix}
%     \begin{bmatrix}
%         \mathbf R_s \\
%         \mathbf R_p
%     \end{bmatrix}
%     % \\\quad\\
%     % \begin{align*}
%     =
%     \begin{bmatrix}
%     \mathbb W & \mathbb {W X} \\
%     \mathbb V & -\mathbb {V X}
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbb {W X} & \mathbb W \\
%     \mathbb {V X} & -\mathbb V
%     \end{bmatrix}^{-1}
%     \begin{bmatrix}
%     \mathbb F \\
%     \mathbb G \\
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbf T_s \\ \mathbf T_p
%     \end{bmatrix},
%     % \end{align*}
% \end{align}

% Since we have four matrix equations for four unknown coefficients ($\mathbf R_s, \mathbf R_p, \mathbf T_s, \mathbf T_p$), they can be derived and used for calculating diffraction efficiencies (also called the reflectance and transmittance).


==> sections/meent_framework/bin/rcwa1.tex <==
% It includes many steps and derivations which cannot be written here due to its size and need for domain knowledge.
% so for readers who is interested in physics, refer this and that.

% This process involves couple of mathematical techniques that scientific ML researchers are familiar with and interested in. For this reason,
% Meent can be a great tool to develop and verify their ideas since RCWA encompasses interesting mathematical techniques such as Fourier analysis, convolution, eigendecomposition, etc., that are favorable topics in scientific ML community. One may try to replace or enhance these steps with machine learning. We will briefly mention them here.

% It includes many steps and derivations which cannot be written here due to its size and need for domain knowledge.
% so we will explain bit more but as less as possible, and for readers who is interested in physics, refer this and that.

Meent uses RCWA for EM solver. It is fast algorithm to calculate the optical characteristics of environment. Due to its space change, it incorporates many skills that needs domain knowledge. Full derivation is huge so see appendix.

In one sentence, RCWA is a technique used to solve partial differential equations (PDEs), notably Maxwell's equations, in Fourier space, aiming to estimate optical properties like diffraction efficiency or field distribution, emerging from the interaction between light and its environment.

This process involves couple of mathematical techniques such as Fourier analysis, convolution, eigendecomposition, etc., that are favorable topics in scientific ML community. For this reason,
Meent can be a great tool to develop and verify their ideas. One may try to replace or enhance these steps with machine learning. 


We will introduce two most important steps that may attract ML researchers - Fourier analysis and eigendecomposition.

\paragraph{Fourier analysis}
%% original
% This is used many times in computer vision because it can capture the important features only with much smaller data size and handle the noises. In SciML community, it's getting hot after zongyi showed her work on Neural operators with FT. This applies RCWA as well. The simulation can be done is a more compressive way than other EM simulation algorithms such as FDTD and FEM. 

This technique is widely employed in computer vision due to its ability to compress the data - capture essential features and effective noise handling \cite{}. 
One successful example in sciML community is Fourier neural operator (FNO) \cite{} which uses Fourier analyses. \textcolor{blue}{write more}.
This concept extends to RCWA, where simulations can be conducted in a more efficient manner (under some constraints) compared to other EM simulation algorithms such as finite-difference time-domain and finite element method.

Simply, Fourier analysis can be expressed as:
\begin{align}\label{eqn:fourier_series_truncation}
    f(x, y) \simeq \sum_{m=-M}^{M} \sum_{n=-N}^{N} c_{n,m} \cdot \exp{\left[j \cdot 2\pi \left(\frac{x}{\Lambda_x}m + \frac{y}{\Lambda_y}n\right)\right]},
\end{align}
where $\Lambda_x$ and $\Lambda_y$ are the period, $c_{n,m}$ is the Fourier coefficients, and $M$ and $N$ are the Fourier truncation order (FTO) in the X and Y direction, respectively. In ML terms, $M$ and $N$ are hyperparameters that affects the simulation accuracy.

\textbf{Eigendecomposition}

% Playing around with \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} results in second order matrix equation

% Fourier analysis, then, takes input \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} and rewrite these in Fourier space. These rewritten 2 equations are combined into a single set of second order equations to find general solution.

% Eig is used to find general solution. Eqs. \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} 

% To find the field, Eqs. \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} are sent to Fourier space, and combined into a single set of second order equations as:

% Electric and magnetic field that sent to Fourier space now can be combined to a single set of second order equations

% \begin{align}
%     \label{eqn:curlyS-omega_LR}
%     (-j\tilde{k}_{g,z})^2
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
%     \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
%     \end{bmatrix}
%     =
%     \boldsymbol{{\Omega}}_{g,LR}^2
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
%     \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
%     \end{bmatrix},
% \end{align}
% where
% \begin{align}
%     \label{eqn:omega_LR}
%     \boldsymbol{{\Omega}}_{g,LR}^2 =
%     \begin{bmatrix}
%     {\tilde{\mathbf K}_y}^2 + (\tilde{\mathbf{K}}_x \llbracket\varepsilon_{r,g}\rrbracket^{-1} \tilde{\mathbf{K}}_x - \mathbf{I}) \llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1} 
%     & \tilde{\mathbf K}_x(\llbracket\varepsilon_{r,g}\rrbracket^{-1}\tilde{\mathbf K}_y\llbracket\varepsilon_{r,g}\rrbracket - \tilde{\mathbf K}_y) \\
%     \tilde{\mathbf K}_y(\llbracket\varepsilon_{r,g}\rrbracket^{-1}\tilde{\mathbf K}_x\llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1} - \tilde{\mathbf K}_x) 
%     & {\tilde{\mathbf K}_x}^2 + (\tilde{\mathbf{K}}_y \llbracket\varepsilon_{r,g}\rrbracket^{-1} \tilde{\mathbf K}_y - \mathbf{I})\llbracket\varepsilon_{r,g}\rrbracket
%     \end{bmatrix}.
% \end{align}
% This omega matrix is composed of wavevector matrices and permittivity map in Fourier space. $\llbracket\ \rrbracket$ is the convolution (a.k.a Toeplitz) matrix: $\llbracket\varepsilon_{r,g}\rrbracket$ and $\llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1}$ are convolution matrices composed of Fourier coefficients of permittivity and one-over-permittivity (by the inverse rule presented in \cite{Li:96} and \cite{Li:hal-00985928}).
This is used to find general solution 
This is simply
% \(Q \Lambda^2 = \Omega^2 Q\)
\begin{align}
    \label{eqn:eigendecomposition}
    \boldsymbol{Q}
    \boldsymbol{\Lambda}^2
    =
    \boldsymbol{\Omega}^2
    \boldsymbol{Q}
\end{align}
that can be solved with eigendecomposition.
Recently there are studies that using ML to find eigenvalues [] []. But those are limited to hermitian cases while ours is non-hermitian.
Here Ex and Ey can be found by eigendecomposition. This is the most time-consuming part in RCWA and a hurdle to adopt GPU as a main device for RCWA. To save time, there have been many researched trying to replace this with NN. Some showed great performance but they were on hermitian matrices while ours is non-hermitian.

% \textbf{Boundary condition} Like PDEs in PINN have boundary conditions, RCWA is also applied. Let's say there are two layers that facing each other. E field of the first layer at the boundary should be matched to the E field of the second layer at the boundary. H field as well, and this can be written in matrix form

% \begin{align}
%     \label{eq:bc}
%     \begin{bmatrix}
%         \sin\psi\ \boldsymbol\delta_{00} \\
%         \cos\psi\ \cos\theta\ \boldsymbol\delta_{00}
%          \\
%         j\sin\psi\ \mathtt n_{\text{I}} \cos\theta\ \boldsymbol\delta_{00} \\
%         -j\cos\psi\ \mathtt n_{\text{I}}\ \boldsymbol\delta_{00} \\
%     \end{bmatrix}
%     +
%     \begin{bmatrix}
%         \mathbf I & \mathbf 0 \\
%         \mathbf 0 & -j\mathbf Z_I \\
%         -j\mathbf Y_I & \mathbf 0 \\
%         \mathbf 0 & \mathbf I
%     \end{bmatrix}
%     \begin{bmatrix}
%         \mathbf R_s \\
%         \mathbf R_p
%     \end{bmatrix}
%     % \\\quad\\
%     % \begin{align*}
%     =
%     \begin{bmatrix}
%     \mathbb W & \mathbb {W X} \\
%     \mathbb V & -\mathbb {V X}
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbb {W X} & \mathbb W \\
%     \mathbb {V X} & -\mathbb V
%     \end{bmatrix}^{-1}
%     \begin{bmatrix}
%     \mathbb F \\
%     \mathbb G \\
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbf T_s \\ \mathbf T_p
%     \end{bmatrix},
%     % \end{align*}
% \end{align}

% Since we have four matrix equations for four unknown coefficients ($\mathbf R_s, \mathbf R_p, \mathbf T_s, \mathbf T_p$), they can be derived and used for calculating diffraction efficiencies (also called the reflectance and transmittance).


==> sections/meent_framework/bin/rcwa2.tex <==
Meent uses RCWA for EM solver. It is fast algorithm to calculate the optical characteristics of environment. Due to its space change, it incorporates many skills that needs domain knowledge. Full derivation is huge so see appendix.

In one sentence, RCWA is a technique used to solve partial differential equations (PDEs), notably Maxwell's equations, in Fourier space, aiming to estimate optical properties like diffraction efficiency or field distribution, emerging from the interaction between light and its environment.

% This process involves couple of mathematical techniques such as Fourier analysis, convolution, eigendecomposition, etc., that are favorable topics in scientific ML community. For this reason,
% Meent can be a great tool to develop and verify their ideas. One may try to replace or enhance these steps with machine learning. 

It includes many steps and derivations which cannot be written here due to its size and need for domain knowledge.
so we will explain bit more but as less as possible, and for readers who is interested in physics, refer this and that.


RCWA is founded on Maxwell's 3rd and 4th equations,
\begin{equation}
    \label{eqn:maxwell 3 and 4}
    \nabla \times \mathbf E = -j\omega\mu_0\mathbf H, \qquad
    \nabla \times \mathbf H = j\omega\varepsilon_0\varepsilon_r\mathbf E,
\end{equation}
where $\mathbf E$ and $\mathbf H$ are electric and magnetic field in real space, $\omega$ denotes the angular frequency, $\mu_0$ is vacuum permeability, $\varepsilon_0$ is vacuum permittivity, and $\varepsilon_r$ is relative permittivity.

These are sent to Fourier space and combined into a single set of second-order matrix equations as:
\begin{align}
    \label{eqn:curlyS-omega_LR}
    (-j\tilde{k}_{g,z})^2
    \begin{bmatrix}
    \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
    \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
    \end{bmatrix}
    =
    \boldsymbol{{\Omega}}_{g,LR}^2
    \begin{bmatrix}
    \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
    \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
    \end{bmatrix},
\end{align}
where omega matrix is composed of wavevector matrices and permittivity map in Fourier space. 

From Eq. \eqref{eqn:curlyS-omega_LR}, we can find general solution of S, and U as well by substituting S into Eq \eqref{eqn:maxwell 3 and 4}.
RCWA then finds the coefficients by using the boundary conditions, and returns the final result.


\begin{align}
    \label{eq:bc}
    \begin{bmatrix}
        \sin\psi\ \boldsymbol\delta_{00} \\
        \cos\psi\ \cos\theta\ \boldsymbol\delta_{00}
         \\
        j\sin\psi\ \mathtt n_{\text{I}} \cos\theta\ \boldsymbol\delta_{00} \\
        -j\cos\psi\ \mathtt n_{\text{I}}\ \boldsymbol\delta_{00} \\
    \end{bmatrix}
    +
    \begin{bmatrix}
        \mathbf I & \mathbf 0 \\
        \mathbf 0 & -j\mathbf Z_I \\
        -j\mathbf Y_I & \mathbf 0 \\
        \mathbf 0 & \mathbf I
    \end{bmatrix}
    \begin{bmatrix}
        \mathbf R_s \\
        \mathbf R_p
    \end{bmatrix}
    % \\\quad\\
    % \begin{align*}
    =
    \begin{bmatrix}
    \mathbb W & \mathbb {W X} \\
    \mathbb V & -\mathbb {V X}
    \end{bmatrix}
    \begin{bmatrix}
    \mathbb {W X} & \mathbb W \\
    \mathbb {V X} & -\mathbb V
    \end{bmatrix}^{-1}
    \begin{bmatrix}
    \mathbb F \\
    \mathbb G \\
    \end{bmatrix}
    \begin{bmatrix}
    \mathbf T_s \\ \mathbf T_p
    \end{bmatrix},
    % \end{align*}
\end{align}

Since we have four matrix equations for four unknown coefficients ($\mathbf R_s, \mathbf R_p, \mathbf T_s, \mathbf T_p$), they can be derived and used for calculating diffraction efficiencies (also called the reflectance and transmittance).

---

This technique is widely employed in computer vision due to its ability to compress the data - capture essential features and effective noise handling \cite{}. 
One successful example in sciML community is Fourier neural operator (FNO) \cite{} which uses Fourier analyses. \textcolor{blue}{write more}.
This concept extends to RCWA, where simulations can be conducted in a more efficient manner (under some constraints) compared to other EM simulation algorithms such as finite-difference time-domain and finite element method.

Simply, Fourier analysis can be expressed as:
\begin{align}\label{eqn:fourier_series_truncation}
    f(x, y) \simeq \sum_{m=-M}^{M} \sum_{n=-N}^{N} c_{n,m} \cdot \exp{\left[j \cdot 2\pi \left(\frac{x}{\Lambda_x}m + \frac{y}{\Lambda_y}n\right)\right]},
\end{align}
where $\Lambda_x$ and $\Lambda_y$ are the period, $c_{n,m}$ is the Fourier coefficients, and $M$ and $N$ are the Fourier truncation order (FTO) in the X and Y direction, respectively. In ML terms, $M$ and $N$ are hyperparameters that affects the simulation accuracy.

\textbf{Eigendecomposition}

% Playing around with \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} results in second order matrix equation

% Fourier analysis, then, takes input \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} and rewrite these in Fourier space. These rewritten 2 equations are combined into a single set of second order equations to find general solution.

% Eig is used to find general solution. Eqs. \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} 

% To find the field, Eqs. \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} are sent to Fourier space, and combined into a single set of second order equations as:

% Electric and magnetic field that sent to Fourier space now can be combined to a single set of second order equations

% \begin{align}
%     \label{eqn:curlyS-omega_LR}
%     (-j\tilde{k}_{g,z})^2
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
%     \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
%     \end{bmatrix}
%     =
%     \boldsymbol{{\Omega}}_{g,LR}^2
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
%     \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
%     \end{bmatrix},
% \end{align}
% where
% \begin{align}
%     \label{eqn:omega_LR}
%     \boldsymbol{{\Omega}}_{g,LR}^2 =
%     \begin{bmatrix}
%     {\tilde{\mathbf K}_y}^2 + (\tilde{\mathbf{K}}_x \llbracket\varepsilon_{r,g}\rrbracket^{-1} \tilde{\mathbf{K}}_x - \mathbf{I}) \llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1} 
%     & \tilde{\mathbf K}_x(\llbracket\varepsilon_{r,g}\rrbracket^{-1}\tilde{\mathbf K}_y\llbracket\varepsilon_{r,g}\rrbracket - \tilde{\mathbf K}_y) \\
%     \tilde{\mathbf K}_y(\llbracket\varepsilon_{r,g}\rrbracket^{-1}\tilde{\mathbf K}_x\llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1} - \tilde{\mathbf K}_x) 
%     & {\tilde{\mathbf K}_x}^2 + (\tilde{\mathbf{K}}_y \llbracket\varepsilon_{r,g}\rrbracket^{-1} \tilde{\mathbf K}_y - \mathbf{I})\llbracket\varepsilon_{r,g}\rrbracket
%     \end{bmatrix}.
% \end{align}
% This omega matrix is composed of wavevector matrices and permittivity map in Fourier space. $\llbracket\ \rrbracket$ is the convolution (a.k.a Toeplitz) matrix: $\llbracket\varepsilon_{r,g}\rrbracket$ and $\llbracket\varepsilon_{r,g}^{-1}\rrbracket^{-1}$ are convolution matrices composed of Fourier coefficients of permittivity and one-over-permittivity (by the inverse rule presented in \cite{Li:96} and \cite{Li:hal-00985928}).
This is used to find general solution 
This is simply
% \(Q \Lambda^2 = \Omega^2 Q\)
\begin{align}
    \label{eqn:eigendecomposition}
    \boldsymbol{Q}
    \boldsymbol{\Lambda}^2
    =
    \boldsymbol{\Omega}^2
    \boldsymbol{Q}
\end{align}
that can be solved with eigendecomposition.
Recently there are studies that using ML to find eigenvalues [] []. But those are limited to hermitian cases while ours is non-hermitian.
Here Ex and Ey can be found by eigendecomposition. This is the most time-consuming part in RCWA and a hurdle to adopt GPU as a main device for RCWA. To save time, there have been many researched trying to replace this with NN. Some showed great performance but they were on hermitian matrices while ours is non-hermitian.

% \textbf{Boundary condition} Like PDEs in PINN have boundary conditions, RCWA is also applied. Let's say there are two layers that facing each other. E field of the first layer at the boundary should be matched to the E field of the second layer at the boundary. H field as well, and this can be written in matrix form

% \begin{align}
%     \label{eq:bc}
%     \begin{bmatrix}
%         \sin\psi\ \boldsymbol\delta_{00} \\
%         \cos\psi\ \cos\theta\ \boldsymbol\delta_{00}
%          \\
%         j\sin\psi\ \mathtt n_{\text{I}} \cos\theta\ \boldsymbol\delta_{00} \\
%         -j\cos\psi\ \mathtt n_{\text{I}}\ \boldsymbol\delta_{00} \\
%     \end{bmatrix}
%     +
%     \begin{bmatrix}
%         \mathbf I & \mathbf 0 \\
%         \mathbf 0 & -j\mathbf Z_I \\
%         -j\mathbf Y_I & \mathbf 0 \\
%         \mathbf 0 & \mathbf I
%     \end{bmatrix}
%     \begin{bmatrix}
%         \mathbf R_s \\
%         \mathbf R_p
%     \end{bmatrix}
%     % \\\quad\\
%     % \begin{align*}
%     =
%     \begin{bmatrix}
%     \mathbb W & \mathbb {W X} \\
%     \mathbb V & -\mathbb {V X}
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbb {W X} & \mathbb W \\
%     \mathbb {V X} & -\mathbb V
%     \end{bmatrix}^{-1}
%     \begin{bmatrix}
%     \mathbb F \\
%     \mathbb G \\
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbf T_s \\ \mathbf T_p
%     \end{bmatrix},
%     % \end{align*}
% \end{align}

% Since we have four matrix equations for four unknown coefficients ($\mathbf R_s, \mathbf R_p, \mathbf T_s, \mathbf T_p$), they can be derived and used for calculating diffraction efficiencies (also called the reflectance and transmittance).


==> sections/meent_framework/bin/rcwa3_backup.tex <==
% RCWA was chosen as an EM simulation solver for Meent due to its high throughput and wide spread adoption in real world applications. 

% Meent uses RCWA for EM simulation


% Meent uses RCWA for EM solver. It is fast algorithm to calculate the optical characteristics of environment. Due to its space change, it incorporates many skills that needs domain knowledge. Full derivation is huge so see appendix.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{sections/meent_framework/images/rcwa.png}
    \caption{\ant{RCWA flow diagram.}
    }
    \label{fig:rcwa-flow}
\end{figure}

In one sentence, RCWA is a technique used to solve partial differential equations (PDEs), notably Maxwell's equations, in Fourier space, aiming to estimate optical properties like diffraction efficiency or field distribution, emerging from the interaction between light and its environment.

% Detailed mathematical derivation 

% This includes  and derivations which cannot be written here due to its size and need for domain knowledge.
Here, we will explain with minimal details for readers from ML, and leave the details in appendix[] and arxiv[] for readers looking for fundamentals of RCWA.

RCWA is based on Faraday's law and Amp\'ere's law of Maxwell's equations \cyp{in a linear matter?},
\begin{equation}
    \label{eqn:maxwell 3 and 4}
    \nabla \times \mathbf E = -j\omega\mu_0\mathbf H, \qquad
    \nabla \times \mathbf H = j\omega\varepsilon_0\varepsilon_r\mathbf E,
\end{equation}
where $\mathbf E$ and $\mathbf H$ are electric and magnetic field in real space, $j$ denotes the imaginary unit number, i.e.\ $j^2 = -1$, $\omega$ denotes the angular frequency, $\mu_0$ is vacuum permeability, $\varepsilon_0$ is vacuum permittivity, and $\varepsilon_r$ is relative permittivity.
% 
% sending these to Fourier space and merged to one matrix equation
% \begin{align}
%     \label{eqn:curlyS-omega_LR}
%     \frac{\partial^2}{\partial(z)^2}
%     \begin{bmatrix}
%     \boldsymbol{S}
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%     \boldsymbol{{\Omega}}^2
%     \end{bmatrix} \cdot
%     \begin{bmatrix}
%     \boldsymbol{S}
%     \end{bmatrix},
% \end{align}
% where omega matrix is composed of wavevector matrices and permittivity map in Fourier space, and S and U are electric and magnetic field in Fourier space. 
% This is second order matrix equation that the general solution can be obtained through eigendecomposition.
%Through Fourier analysis, curl becomes multiplication, multiplication becomes convolution, and 
After Fourier transform, $\mathbf E$ and $\mathbf H$ in real space become $\boldsymbol{\mathfrak{S}}$ and $\boldsymbol{\mathfrak{U}}$ in Fourier space, respectively, and Eq. \eqref{eqn:maxwell 3 and 4} then turns into 
\begin{align}
    \label{eqn:maxwell 3 and 4 in fourier space}
    (-j\tilde{k}_{z}) \cdot
    \boldsymbol{\mathfrak{S}}
    =
    \boldsymbol{{\Omega}}_L \cdot
    \boldsymbol{\mathfrak{U}}, \qquad
    (-j\tilde{k}_{z}) \cdot
    \boldsymbol{\mathfrak{U}}
    =
    \boldsymbol{{\Omega}}_R \cdot
    \boldsymbol{\mathfrak{S}},
\end{align} 
where the matrices $\boldsymbol\Omega_L$ and $\boldsymbol\Omega_R$ are composed of wavevector matrices and convolution matrices that lie in Fourier space, $\tilde k_z$ is a normalized wavevector in the $z$-direction.
%and $j$ is imaginary. 
We can find $\boldsymbol{\mathfrak{S}}$ by merging Eq. \eqref{eqn:maxwell 3 and 4 in fourier space} in a single matrix equation as
% Merging these into a single matrix equation results in
% 
% Then transform combining the transformed two equs in eq 1 makes this equation
% 
% Fourier analysis, then, takes input \eqref{eqn:maxwell 3} and \eqref{eqn:maxwell 4} and rewrite these in Fourier space, as S and U.
% \begin{align}
%     \label{eqn:Eg-curly S}
%     \mathbf{E}_{g}(x,y,z) &= \sum_{m=-M}^{M} \sum_{n=-N}^{N} \boldsymbol{\mathfrak{S}}_{g,(n,m)} \cdot e^{-j(k_{x,m}x + k_{y,n}y + k_{g,z}z)}, \\
%     \label{eqn:Hg-curly U}
%     \mathbf{H}_{g}(x,y,z) &= \sum_{m=-M}^{M} \sum_{n=-N}^{N} \boldsymbol{\mathfrak{U}}_{g,(n,m)} \cdot e^{-j(k_{x,m}x + k_{y,n}y + k_{g,z}z)},
% \end{align}
% 
% These rewritten 2 equations are combined into a single set of second order equations to find general solution.
% Then eq 1 becomes 
% \begin{align}
%     \label{eqn:curlyS-omega_LR}
%     (-j\tilde{k}_{z})^2 \cdot
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%     \boldsymbol{{\Omega}}^2
%     \end{bmatrix} \cdot
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}
%     \end{bmatrix},
% \end{align}
\begin{align}
    \label{eqn:curlyS-omega_LR}
    (-j\tilde{k}_{z})^2 \cdot
    \boldsymbol{\mathfrak{S}}
    =
    \boldsymbol{{\Omega}}_{LR}^2 \cdot
    \boldsymbol{\mathfrak{S}}, \qquad
    % where \quad \boldsymbol\Omega_{LR}^2=\boldsymbol\Omega_{L}\cdot\boldsymbol\Omega_{L}.
\end{align}
where the matrix $\boldsymbol\Omega_{LR}^2$ is a matrix product of $\boldsymbol\Omega_{L}$ and $\boldsymbol\Omega_{R}$.
% 
% These rewritten 2 equations are combined into a single set of second order equations to find general solution.
% \begin{align}
%     \label{eqn:curlyS-omega_LR}
%     (-j\tilde{k}_{z})^2
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}_{\vec x} \\
%     \boldsymbol{\mathfrak{S}}_{\vec y}
%     \end{bmatrix}
%     =
%     \boldsymbol{{\Omega}}_{LR}^2
%     \begin{bmatrix}
%     \boldsymbol{\mathfrak{S}}_{\vec x} \\
%     \boldsymbol{\mathfrak{S}}_{\vec y}
%     \end{bmatrix},
% \end{align}
% where omega matrix is composed of wavevector matrices and permittivity map in Fourier space. 
% 
% this has a general form of eigendecomposition: S for eigenvectors and (-jkz) for eigenvalues of the matrix omega.
% 
% This has a form of
% \(\boldsymbol{Q}\boldsymbol{\Lambda}^2 = \boldsymbol{\Omega}^2 \boldsymbol{Q},\) that can be addressed through eigendecomposition, enabling the derivation of the solutions for S. By substituting the resultant solution for S into equation 1, a solution for U can be obtained.
% 
% RCWA then finds the coefficients by using the boundary conditions. Then we can find the particular solution of S and U. 
% 
As the form implies, this equation can be solved by finding the eigendecomposition of $\boldsymbol\Omega_{LR}^2$ and obtaining the eigenvectors $\boldsymbol{\mathfrak{S}}$ and the eigenvalues $(-j\tilde{k}_{z})$. Then by substituting the eigenvectors for $\boldsymbol{\mathfrak{S}}$ in Eq. \eqref{eqn:maxwell 3 and 4 in fourier space}, the corresponding solution of $\boldsymbol{\mathfrak{U}}$ can be obtained.

% This equation has a form of eigendecomposition: applying eigendecomposition to the matrix $\Omega$ returns the eigenvalues and eigenvectors $(-j\tilde{k}_{z})$.

% The presented equation takes the form \(\boldsymbol{Q}\boldsymbol{\Lambda}^2 = \boldsymbol{\Omega}^2 \boldsymbol{Q},\) which can be resolved through eigendecomposition, facilitating the derivation of solutions for $\boldsymbol{\mathfrak{S}}$. Subsequently, substituting $\boldsymbol{\mathfrak{S}}$ into equation 1, a corresponding solution for $\boldsymbol{\mathfrak{U}}$ can be obtained.


% $\boldsymbol{\mathfrak{S}}$ and $\boldsymbol{\mathfrak{U}}$, what we just calculated, are the set of modes allowed to exist in given matter. To see the interaction with the light, boundary conditions are used to decide the weights of each mode.
% These weights, or coefficients, describes how each pattern affects the distribution of light. and specifically coefficients at the input and output terminal are called diffraction efficiencies, the primary purpose of RCWA.
% The fields in real space can be reconstructed with inverse transform.

$\boldsymbol{\mathfrak{S}}$ and $\boldsymbol{\mathfrak{U}}$, which we have just computed, represent the permissible modes within a given medium.
To understand their interaction with incoming and outgoing light, we employ boundary conditions to ascertain their respective weights of the modes, or in other words, the coefficients in linear combination of the modes. These coefficients describe the extent of each mode's influence on the overall field distribution. 
Notably, coefficients at the input and output interfaces are designated as diffraction efficiencies, also called the reflectance and transmittance, serving as the primary purpose of RCWA.
Subsequently, the inverse transformation from Fourier space to real space enables the reconstruction of the field distribution.


% These fields have to be weighed to satisfy the boundary conditions. Consequently, the particular solutions for both $\boldsymbol{\mathfrak{S}}$ and $\boldsymbol{\mathfrak{U}}$ can be determined, and able to find the diffraction efficiencies. One more step is to inverse transform of the fields from Fourier to real, called Field reconstruction.

% \begin{align}
%     \label{eq:bc}
%     \begin{bmatrix}
%         \sin\psi\ \boldsymbol\delta_{00} \\
%         \cos\psi\ \cos\theta\ \boldsymbol\delta_{00}
%          \\
%         j\sin\psi\ \mathtt n_{\text{I}} \cos\theta\ \boldsymbol\delta_{00} \\
%         -j\cos\psi\ \mathtt n_{\text{I}}\ \boldsymbol\delta_{00} \\
%     \end{bmatrix}
%     +
%     \begin{bmatrix}
%         \mathbf I & \mathbf 0 \\
%         \mathbf 0 & -j\mathbf Z_I \\
%         -j\mathbf Y_I & \mathbf 0 \\
%         \mathbf 0 & \mathbf I
%     \end{bmatrix}
%     \begin{bmatrix}
%         \mathbf R_s \\
%         \mathbf R_p
%     \end{bmatrix}
%     % \\\quad\\
%     % \begin{align*}
%     =
%     \begin{bmatrix}
%     \mathbb W & \mathbb {W X} \\
%     \mathbb V & -\mathbb {V X}
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbb {W X} & \mathbb W \\
%     \mathbb {V X} & -\mathbb V
%     \end{bmatrix}^{-1}
%     \begin{bmatrix}
%     \mathbb F \\
%     \mathbb G \\
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbf T_s \\ \mathbf T_p
%     \end{bmatrix},
%     % \end{align*}
% \end{align}

% Since we have four matrix equations for four unknown coefficients ($\mathbf R_s, \mathbf R_p, \mathbf T_s, \mathbf T_p$), they can be derived and used for calculating diffraction efficiencies (also called the reflectance and transmittance).


==> sections/meent_framework/bin/rcwa_backup.tex <==
RCWA is founded on Maxwell's 3rd and 4th equations,
\begin{equation}
    \label{eqn:maxwell 3 and 4}
    \nabla \times \mathbf E = -j\omega\mu_0\mathbf H, \qquad
    \nabla \times \mathbf H = j\omega\varepsilon_0\varepsilon_r\mathbf E,
\end{equation}
where $\mathbf E$ and $\mathbf H$ are electric and magnetic field in real space, $\omega$ denotes the angular frequency, $\mu_0$ is vacuum permeability, $\varepsilon_0$ is vacuum permittivity, and $\varepsilon_r$ is relative permittivity.

These are sent to Fourier space and combined into a single set of second-order matrix equations as:
\begin{align}
    \label{eqn:curlyS-omega_LR}
    (-j\tilde{k}_{g,z})^2
    \begin{bmatrix}
    \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
    \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
    \end{bmatrix}
    =
    \boldsymbol{{\Omega}}_{g,LR}^2
    \begin{bmatrix}
    \boldsymbol{\mathfrak{S}}_{g,\vec x} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}} \\
    \boldsymbol{\mathfrak{S}}_{g,\vec y} \cdot e^{-j\tilde{k}_{g,z}\tilde{z}}
    \end{bmatrix},
\end{align}
where omega matrix is composed of wavevector matrices and permittivity map in Fourier space. 

From Eq. \eqref{eqn:curlyS-omega_LR}, we can find general solution of S, and U as well by substituting S into Eq \eqref{eqn:maxwell 3 and 4}.
RCWA then finds the coefficients by using the boundary conditions, and returns the final result.


\begin{align}
    \label{eq:bc}
    \begin{bmatrix}
        \sin\psi\ \boldsymbol\delta_{00} \\
        \cos\psi\ \cos\theta\ \boldsymbol\delta_{00}
         \\
        j\sin\psi\ \mathtt n_{\text{I}} \cos\theta\ \boldsymbol\delta_{00} \\
        -j\cos\psi\ \mathtt n_{\text{I}}\ \boldsymbol\delta_{00} \\
    \end{bmatrix}
    +
    \begin{bmatrix}
        \mathbf I & \mathbf 0 \\
        \mathbf 0 & -j\mathbf Z_I \\
        -j\mathbf Y_I & \mathbf 0 \\
        \mathbf 0 & \mathbf I
    \end{bmatrix}
    \begin{bmatrix}
        \mathbf R_s \\
        \mathbf R_p
    \end{bmatrix}
    % \\\quad\\
    % \begin{align*}
    =
    \begin{bmatrix}
    \mathbb W & \mathbb {W X} \\
    \mathbb V & -\mathbb {V X}
    \end{bmatrix}
    \begin{bmatrix}
    \mathbb {W X} & \mathbb W \\
    \mathbb {V X} & -\mathbb V
    \end{bmatrix}^{-1}
    \begin{bmatrix}
    \mathbb F \\
    \mathbb G \\
    \end{bmatrix}
    \begin{bmatrix}
    \mathbf T_s \\ \mathbf T_p
    \end{bmatrix},
    % \end{align*}
\end{align}

Since we have four matrix equations for four unknown coefficients ($\mathbf R_s, \mathbf R_p, \mathbf T_s, \mathbf T_p$), they can be derived and used for calculating diffraction efficiencies (also called the reflectance and transmittance).

% original
This process involves couple of mathematical techniques that scientific ML researchers are familiar with and interested in. For this reason,
Meent can be a great tool to develop and verify their ideas since RCWA encompasses interesting mathematical techniques such as Fourier analysis, convolution, eigendecomposition, etc., that are favorable topics in scientific ML community. One may try to replace or enhance these steps with machine learning. We will briefly mention them here.

Meent is an integration of these implementations in a modularized manner, inviting researchers to experiment with ML methods.

For example, researchers may explore the potential of ML to replace or enhance these steps which will be briefly introduced here.


==> sections/meent_framework/potential.tex <==

Recently there are studies that using ML to find eigenvalues [] []. But those are limited to hermitian cases while ours is non-hermitian.
Here Ex and Ey can be found by eigendecomposition. This is the most time-consuming part in RCWA and a hurdle to adopt GPU as a main device for RCWA. To save time, there have been many researched trying to replace this with NN. Some showed great performance but they were on hermitian matrices while ours is non-hermitian.

